Feasibility of hybrid inverse problems in limited view

Hybrid inverse problems such as Acousto-Electric Tomography, Current Density Imaging or Magnetic Resonance Electric Impedance Tomography are concerned with reconstructing the electrical conductivity from interior measurements. For a two-dimensional object the measurements correspond to two different functions imposed as the Neumann boundary condition to an elliptic PDE. In limited view these functions are only non-zero on the part of the boundary that one can control. In this paper we address how to choose such boundary functions in limited view such that the reconstruction procedure is feasible. This is related to the corresponding Jacobian being non-zero. We supplement the theoretical results by numerical reconstructions following the approach of Acousto-Electric Tomography.

==> Text.tex <==

{\color{red} Ideas:
\begin{enumerate}
    \item Numerical results:
    \begin{itemize}
        \item Use $\Omega=B(0,1)$ and the unit normal $(\cos(\eta(t)),\sin(\eta(t)))$ adapted to the interval $[\eta(0), \eta(\ell)]$ as examples of boundary functions for which $\gamma(0)=\gamma(\ell)$ and $\abs{\mathrm{Ind}(\gamma)}=1$. Use then cut offs of $(\cos(\eta(t)),\sin(\eta(t)))$ adapted by constants so that they integrate to zero as examples of boundary functions for which $\gamma(0)\neq\gamma(\ell)$ and $\abs{\mathrm{Ind}(\gamma)}<1$
        \item The less oscillating boundary functions do perform slightly worse for a smaller boundary of control: "mini" and "sma", but actually perform a bit better for "SmaMed" and "Med"
        \item The more oscillating boundary functions induce more jumps between $-\pi$ and $\pi$ for $\theta$ these can be adapted, but might induce small artifacts in the reconstruction (especially in the presence of noise)
        \item In the presence of noise the less oscillating functions actually perform a bit better for $\Gamma_{med}$. This could be, because for the more oscillating functions there is this jump in $\theta$ and furthermore, the more oscillating functions already performed worse in this case for no noise
        \item For "Lar" and "Sma" the more oscillating functions tend to work better in the presence of noise 
        \item For the less oscillating functions the lower bound of the eigenvalues discards more information than in the more oscillating function case, since the values of the Jacobian simply are smaller in the less oscillating function case. This might be due to the fact that in the more oscillating function case the current is forced to stream further into the domain than for less oscillating boundary functions?
    \end{itemize}


    \item Ideas to prove under which circumstances the coordinates of the unit normal work as boundary functions for which the corresponding solutions have a non-vanishing Jacobian in the full view setting:
\begin{itemize}
    \item One can proof that $\abs{\mathrm{Ind}(\nu)}=1$ if $\eta(t)=\partial \Omega$ defines a plane, regular, simple, closed curve since by "Theorem 2 in DoCarmo, Differential geometry of curves and surfaces, Section 5-7" the rotation index of $\partial \Omega$ so the winding number of $\dot{\eta}$ is +1 or -1. As $\dot{\eta}$ is simply the tangent vector which is orthogonal to the unit normal it follows that $\abs{\mathrm{Ind}(\nu)}=1$. The unit normal is then simply $\nu(t)=\frac{(\eta_2'(t),-\eta_1'(t))}{\norm{\dot{\eta}(t)}}$. Note that the coordinates of the unit tangent work equally well as a choice of the boundary functions. However, the unit normal is a more obvious choice as the pair of boundary functions $(\nu_1,\nu_2)$ yields
    \begin{equation*}
        \nabla u_1 \cdot \nu = \nu_1, \quad \nabla u_2 \cdot \nu = \nu_2.
    \end{equation*}
    Hence, when $\sigma = 1$ the choice $(f_1,f_2)=(\nu_1,\nu_2)$ yields the solution $(u_1,u_2)=(x_1,x_2)$ to the PDE similar to the choice $(f_1,f_2)=(x_1,x_2)$ in the Dirichlet setting. 
    \item In the case that $\partial \Omega$ is convex it follows that $\gamma(t)=(f^1(\eta(t)),f^2(\eta(t)))$ satisfies $\arg(\gamma(t))$ is monotone (as there are no indents that yield local minima or maxima)
    \item In the case that $\partial \Omega$ is convex and has two orthogonal symmetry axes it follows that $\int_{\partial \Omega} \nu_1 \mathrm{d}S=\int_{\partial \Omega} \nu_2 \mathrm{d}S=0$ since in this case each integral can be split into two parts $\Gamma_1,\Gamma_2$ so that $\int _{\Gamma_1}\nu_i \mathrm{d}S=-\int _{\Gamma_2}\nu_i \mathrm{d}S$ respectively.
\end{itemize}
    \item Maybe one can do a direct generalization of the Rado-Kneser-Choquet Theorem as done in "Bauman, Patricia; Marini, Antonella; Nesi, Vincenzo: Univalent solutions of an elliptic system of partial differential equations arising in homogenization (2001)" (check also the reference: "Giovanni Alessandrini, Vincenzo Nesi: Univalent σ-Harmonic Mappings")?:
    \begin{itemize}
        \item In the full view setting with Dirichlet conditions: Can the Brouwer degree of the homeomorphism $\Phi$ be thought of the winding number of $\Psi=\Phi \vert_{\partial \Omega}$ that has to be one? Furthermore, that $\Phi$ has to map from the boundary of $\Omega$ to the boundary of a convex domain $\Delta$ does that correspond to that $\arg(\dot{\gamma}(t))$ has to be monotone?
        \item Can the full view setting results be obtained in a similar manner with Neumann conditions?: So that now the Neumann data has to satisfy $\int_{\partial \Omega} \phi^1 dS=\int_{\partial \Omega} \phi^2 dS=0$, but again $\Phi$ has to be a homeomorphism that hat Brouwer degree one (as the Index of $\Psi$ has to be one)? And similarly that $\Phi$ has to map to the boundary of a convex domain so that $\arg(\gamma(t))$ is monotone?
        \item Can these results be generalized to the limited view settings, where $\Psi=\Phi \vert_{\Gamma}$ and $\Psi$ maps to a part of the boundary of a convex domain, so that $\arg(\dot{\gamma}(t))$ and $\arg(\gamma(t))$ respectively are still monotone?
    \end{itemize}
    \item Note that in the full view setting when $\eta(t)=\partial \Omega$ defines a plane, regular, simple, closed curve it follows that both $\abs{\mathrm{Ind}(\eta)}=1$ and $\abs{\mathrm{Ind}(\dot{\eta})}=1$
\end{enumerate}
}

\section{Introduction}
In 1980 A.P.Calderón proposed the inverse problem whether it is possible to recover the electrical conductivity by making voltage and current measurements at the boundary. This procedure is today known as electrical impedance tomography (EIT). Since the 1980s there has been an increasing interest in inverse problems dealing with the reconstruction of electrical conductivities. In this paper we focus on hybrid inverse problems that consists of two steps: First combine the EIT approach with another method so that interior measurements can be obtained; secondly recover the conductivity from the interior measurements. We focus on applications that combine the EIT approach with magnetic resonance imaging (MRI) or a



\section{Main results}

We state the following proposition without proof corresponding to \cite[Thm 2.8]{AlessandriniMagnanini94}.
\begin{proposition}\label{prop:am94}
    Let $\Omega \subset \R^2$ be a simply connected bounded Lipschitz domain and let $\sigma \in L^{\infty}(\overline{\Omega})$ satisfy \eqref{ellip}. Let $g \in H^{-\frac{1}{2}}(\partial \Omega)$ with $\int_{\partial \Omega} g \, \mathrm{d}S=0$ and $u \in H^1(\Omega)$ be a nonconstant solution of 
\begin{equation*}
\begin{cases}
    -\mathrm{div}(\sigma \nabla u)=0 & \text{in }\Omega,\\
    \sigma \nabla u \cdot \nu = g & \text{on }\partial \Omega.
\end{cases}
\end{equation*}
Denote by $2M$ the number of closed arcs $\Gamma_1,...,\Gamma_{2M}$ into which $\partial \Omega$ can be split for which $(-1)^j g\geq 0$ on $\Gamma_j$, $j=1,...,2M$. Then the number of interior critical points $N$ satisfies:
\begin{equation*}
    N \leq M - 1.
 \end{equation*}
\end{proposition}

\begin{lemma}\label{lem:4points}
    Let $\Omega, \sigma, u$ and $g$ be as in proposition \ref{prop:am94}. By the proposition it follows that when $\Omega$ has one critical point $x_0 \in \Omega$ so that $\nabla u(x_0)=0$ then $\partial \Omega$ must be composed of at least 4 closed arcs $\Gamma_1, \Gamma_2, \Gamma_3, \Gamma_4$ for which $(-1)^j g \geq 0$. Hence, there must exist points $x_1 \in \Gamma_1, x_2 \in \Gamma_2, x_3 \in \Gamma_3$ and $x_4 \in \Gamma_4$ such that
    \[
\sigma \nabla u \cdot \nu \vert_{x=x_1} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_2} > 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_3} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_4} > 0.\]
\end{lemma}

Let $\gamma: [0,\ell] \to \R^2$ be a $C^1$ curve (we do not require that $\gamma(0) = \gamma(\ell)$). We say that $\gamma$ is regular if $\dot{\gamma}(t) \neq 0$ for all $t \in [0,\ell]$. For a regular curve, we may write a polar coordinate representation for $\gamma(t)$ as 
\[
\gamma(t) = r(t) e^{i\phi(t)}
\]
where $r(t) = \abs{\gamma(t)}$ and $\phi(t)$ are continuous functions in $[0,\ell]$. The function 
\[
\mathrm{arg}(\gamma(t)) := \phi(t)
\]
is well defined modulo a constant in $2\pi \mathbb{Z}$. We define 
\[
\mathrm{Ind}(\gamma) := \frac{\mathrm{arg}(\gamma(\ell)) - \mathrm{arg}(\gamma(0))}{2\pi}.
\]
If $\gamma$ is closed, i.e.\ $\gamma(0) = \gamma(\ell)$, then $\mathrm{Ind}(\gamma)$ is the winding number of the curve $\gamma(t)$, which is an integer. If $\gamma$ is not closed but $\mathrm{arg}(\dot{\gamma}(t))$ is monotone (i.e.\ nondecreasing or nonincreasing), we may still interpret $\mathrm{Ind}(\dot{\gamma})$ as the winding number of $\dot{\gamma}(t)$, and this is then a real number.

We now give sufficient conditions on a pair of boundary data vanishing outside an arc $\Gamma$ such that the corresponding solutions $u_1, u_2$ satisfy $\mathrm{det} [\nabla u_1(x) \, \nabla u_2(x)]\neq 0$ everywhere in $\Omega$. Condition (a) below is related to the case where $u_i|_{\partial \Omega}$ are continuous and condition (b) allows discontinuous boundary data. Note that part (a) can be seen as a consequence of \cite[Theorem 2.7]{AlessandriniMagnanini94}, while for part (b) Proposition \ref{PropNoCriticalPoints} is needed.

\begin{theorem}\label{thm:Main}
Let $\Omega \subset \R^2$ be a bounded simply connected domain with $C^1$ boundary curve $\eta: [0,2\pi] \to \partial \Omega$, and let $\sigma \in L^{\infty}(\overline{\Omega};\R^{2\times 2})$ satisfy \eqref{ellip}. Let $\Gamma = \eta([0,\ell])$ be a closed arc in $\partial \Omega$. Let $f_1, f_2 \in C^1(\Gamma)$ be linearly independent so that $\int_{\Gamma} f_1 \,\mathrm{d}S=\int_{\Gamma} f_2 \,\mathrm{d}S=0$‚ and assume that $u_i$ is the unique solution of 
\begin{equation}\label{bvpui}
    \begin{cases}
        -\mathrm{div}(\sigma \nabla u_i)=0 & \text{in }\Omega,\\
        \sigma \nabla u_i \cdot \nu=f_i & \text{on }\Gamma ,\\
        \sigma \nabla u_i \cdot \nu = 0 & \text{on }\partial \Omega \backslash \Gamma.
    \end{cases}
\end{equation}
Assume that the curve $\gamma: [0,\ell] \to \R^2$, $\gamma(t) = (f_1(\eta(t)), f_2(\eta(t)))$ is regular, $\gamma(t) \neq 0$ for all $t \in [0,\ell]$,  and that one of the following holds:
\begin{enumerate}
    \item[(a)] $\gamma(0)=\gamma(\ell)$, and $\mathrm{arg}(\gamma(t))$ is monotone, and $\abs{\mathrm{Ind}(\gamma)} < 1$; or 
    \item[(b)] $\gamma(0)\neq \gamma(\ell)$, and $\mathrm{arg}(\gamma(t))$ is monotone, and $\abs{\mathrm{Ind}(\gamma)} \leq 1$
\end{enumerate}
Then $\mathrm{det} [\nabla u_1(x) \, \nabla u_2(x)]\neq 0$ for all $x \in \Omega$.

\end{theorem}

%\begin{theorem}\label{thm:Main}
%Let $\Omega \subset \R^2$ be a bounded simply connected domain with $C^1$ boundary curve $\eta: [0,2\pi] \to \partial \Omega$, and let $\sigma \in C^{0,\alpha}(\overline{\Omega};\R^{2\times 2})$ satisfy \eqref{ellip}. Let $\Gamma = \eta([0,\ell])$ be a closed arc in $\partial \Omega$. Let $f_1, f_2 \in C^1(\Gamma)$ be linearly independent‚ and assume that $u_i$ is the unique solution of 
%\begin{equation}\label{bvpui}
%    \begin{cases}
%        -\mathrm{div}(\sigma \nabla u_i)=0 & \text{in }\Omega,\\
%        \sigma \nabla u_i \cdot \nu=f_i & \text{on }\Gamma ,\\
%        \sigma \nabla u_i \cdot \nu = 0 & \text{on }\partial \Omega \backslash \Gamma.
%    \end{cases}
%\end{equation}
%Assume that the curve $\gamma: [0,\ell] \to \R^2$, $\gamma(t) = (f_1(\eta(t)), f_2(\eta(t)))$ is regular,  and that one of the following holds:
%\begin{enumerate}
%    \item[(a)] $\sigma \nabla u_i \cdot \nu\vert_{\partial \Omega}$ are continuous, and $\mathrm{arg}(\gamma(t))$ is monotone, and $\abs{\mathrm{Ind}(\gamma)} \leq 1$; or 
%    \item[(b)] $\sigma \nabla u_i \cdot \nu\vert_{\partial \Omega}$ are continuous at $\eta(0)$, and $\mathrm{arg}(\gamma(t))$ is monotone, and $\abs{\mathrm{Ind}(\gamma)} \leq 1/2$; or
%    \item[(c)] $\sigma \nabla u_i \cdot \nu\vert_{\partial \Omega}$ are continuous at $\eta(0)$, and $\mathrm{arg}(\dot{\gamma(t)})$ is monotone, and $\abs{\mathrm{Ind}(\dot{\gamma})} \leq 1/2$.
%\end{enumerate}
%Then $\mathrm{det} [\nabla u_1(x) \, \nabla u_2(x)]\neq 0$ for all $x \in \Omega$.
%
%\end{theorem}
\beginproof
Assume that (a) or (b) holds, but one has $\mathrm{det} [\nabla u_1(x_0) \, \nabla u_2(x_0)] =  0$ for some $x_0 \in \Omega$. Then there is a vector $\vec{\alpha} = (\alpha_1, \alpha_2) \in \R^2 \setminus \{0\}$ such that the function 
\[
u = \alpha_1 u_1 + \alpha_2 u_2
\]
satisfies $\nabla u(x_0) = 0$. Note that if $u$ is a constant, then 
\begin{equation*}
    0=\sigma \nabla u \cdot \nu\vert_{\Gamma} = \alpha_1 \sigma \nabla u_1 \cdot \nu\vert_{\Gamma} + \alpha_2 \sigma \nabla u_2 \cdot \nu\vert_{\Gamma} = \alpha_1 f_1 + \alpha_2 f_2 
\end{equation*}
Hence $f_1$ and $f_2$ would be linearly dependent. Thus, we may assume that $u$ is nonconstant. Note that $\sigma \nabla u_i|_{\partial \Omega} \cdot \nu$ are discontinuous, but piecewise $C^1$ and hence they are in $H^{-\frac{1}{2}}(\partial \Omega)$. Then by Lemma \ref{lem:4points} there exist distinct points $x_1, x_2, x_3, x_4 \in \partial \Omega$ that are in counterclockwise order along $\partial \Omega$ such that 
\[
\sigma \nabla u \cdot \nu \vert_{x=x_1} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_2} > 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_3} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_4} > 0.\]
Consider the function $h: [0,\ell] \to \R$ given by 
\begin{equation}\label{g_fun}
h(t) := \sigma(\eta(t)) \nabla u(\eta(t)) \cdot \nu(\eta(t))= \vec{\alpha} \cdot \gamma(t).
\end{equation}
Extend $h$ by zero to $[0,2\pi)$. Writing $x_j = \eta(t_j)$ where $t_j \in [0,2\pi)$, we have 
\begin{equation} \label{g_contra}
h(t_1) > 0, \quad h(t_2) < 0, \quad h(t_3) > 0, \quad h(t_4) < 0.
\end{equation}
We may assume that $t_1 < t_2 < t_3 < t_4$ (possibly after a cyclic permutation of the indices and after changing $h$ to $-h$).

We now assume that (a) holds, and want to derive a contradiction with \eqref{g_contra}. Since $\gamma(t)\neq 0$, $\mathrm{arg}(\gamma(t))$ is monotone and $\abs{\mathrm{Ind}(\gamma(t))} < \frac{3}{2}$, it follows that $h(t)$ either has at most two zeros in $[0,\ell]$, or has three zeros two of which are at $t=0$ and $t=\ell$. Note that if the argument is not strictly monotone, we make the interpretation that some of these zeros of $h$ could be intervals. Since we assume that $f_1,f_2\in C^1(\Gamma)$ it follows that $h \in C^1(\Gamma)$. Now by \eqref{g_contra} $h$ has a zero in the interval $(t_1,t_2)$, a zero in the interval $(t_2,t_3)$ and a zero in the interval $(t_3,t_4)$. Therefore $h$ has at least three zeros in $(0,\ell)$. This is a contradiction. 
\QEDA

%Assume that (c) holds. One has the formula \eqref{g_fun} for $g(t)$ and the formula \eqref{gprime_formula} for $g'(t)$ on $[0,\ell]$. Since $\mathrm{arg}(\gamma(t))$ is monotone and $\abs{\mathrm{Ind}(\gamma(t))} = 1/2$, $g(t)$ has exactly one zero in $]0,\ell]$. Furthermore, as $\mathrm{arg}(\dot{\gamma}(t))$ is monotone and $\abs{\mathrm{Ind}(\dot{\gamma}(t))} \leq 1$, $g'(t)$ has at most two zeros in $[0,\ell]$, or has three zeros two of which are at $t=0$ and $t=\ell$. Note that the zeros of $g$ and $g'$ could be intervals. By the assumption that $u_i\vert_{\partial \Omega}$ is continuous at $t=0$ it follows that $g(0)=0$, while there may be a discontinuity at $t=\ell$. By the observations in the proof of (b) $g'$ has at least two zeros in $(0,\ell)$. Let us assume that $g'$ has exactly two zeros. If $u(x_0)\geq 0$ then $g$ has either two zeros of which one is in $($

%That $g'$ has at most three zeros (of which two are at the endpoints) and $g$ has at most two zeros (of which one is at $t=0$) is in contradiction with \eqref{g_contra}.
%Assume now that (c) holds. One still has the formula \eqref{gprime_formula} for $g'(t)$ on $[0,\ell]$. Now if $g'(t)$ has no zeros on $[0,\ell]$, then $g$ is strictly increasing and decreasing in $[0,\ell]$, and this is incompatible with \eqref{g_contra}. Suppose then that $g'(t_0) = 0$ for some $t_0 \in [0,\ell]$. By \eqref{gprime_formula} one has $\alpha = c \dot{\gamma}(t_0)^{\perp}$ for some $c \neq 0$. Then on $[0,\ell]$ one has 
%\[
%g(t) = c \dot{\gamma}(t_0)^{\perp} \cdot \gamma(t).
%\]
%By the assumption in (c) we have $g(t) \neq 0$ for all $t \in [0,\ell]$. Since $g = 0$ in $(\ell, 2\pi)$ and since $g'(t)$ can have at most three zeros in $[0,\ell]$ by the assumption $\abs{\mathrm{Ind}(\dot{\gamma})} < 3/2$, we again obtain a contradiction with \eqref{g_contra}.

\begin{remark}
    In the full view setting when $\Gamma=\partial \Omega$ and the domain is convex, the first and second coordinate of the unit vector $(f_1,f_2)=(\nu_1,\nu_2)$ are an example for which Theorem \ref{thm:Main} (a) is satisfied as $\nu$ in this case naturally makes exactly one rotation in counterclockwise direction along the boundary so that $\mathrm{Ind}(\gamma)=1$ and $\arg(\gamma(t))$ is nondecreasing. 
\end{remark}

\begin{remark}
    Denote by $(f_1^\ell,f_2^\ell)$ cut offs of the coordinate functions $(f_1,f_2)=(x_1,x_2)$. Let $\Gamma = \eta([0,\ell])$ be the support of $f_i^\ell$ and $\partial \Omega = \eta([0,2\pi])$ be the support of $f_i$. These cut offs are automatically captured by Theorem \ref{thm:Main} after a normalization so that $\int_{\Gamma} f_1^d \,\mathrm{d}S=\int_{\Gamma} f_2^d \,\mathrm{d}S=0$:
    \begin{equation*}
        f_i^\ell(\eta(t)) = f_i(\eta(t)) \chi_{[0,\ell]}(t) - \frac{\int_{\partial \Omega} f_i(\eta(t)) \chi_{[0,\ell]}(t)}{\ell}
    \end{equation*}
\end{remark}

%\begin{remark}
%Condition (a) in Theorem \label{thm:Main} is equivalent to $\mathrm{arg}(\dot{\gamma}(t))$ being monotone and $\abs{\mathrm{Ind}(\dot{\gamma})}\leq 1$. While the first choice limits the number of nonnegative and nonpositive parts of $\sigma \nabla u_i \cdot \nu$  along the boundary, the second choice limits the number of nonincreasing and nondecreasing parts. By the zero Neumann condition on $\partial \Omega \backslash \Gamma$ the function $\sigma \nabla u_i \cdot \nu\vert_{partial \Omega}$ is forced to be zero at $\eta(0)$ and $\eta(\ell)$. This implies that the number of nonnegative and nonpositive parts and nonincreasing and nondecreasing parts are identical.
%\end{remark}


%\begin{example}
%Let $\Omega$ be the unit disk so that $\eta(t)=\mathrm{argument}(\cos(t)+i\sin(t))$ and consider $\Gamma = \eta([0,\pi/4])$.  
%\begin{itemize}
%    \item The following pair of boundary functions is an example for which condition (b) in Theorem \label{thm:Main} is satisfied but not condition (c): $$(f_1(\eta(t)),f_2(\eta(t)))=(\cos(7t)-1,\sin(4t)).$$ In this case $\mathrm{arg}(\gamma(t))$ is monotone and $$\abs{\mathrm{Ind}(\gamma)}= \frac{1}{2},$$ but $\mathrm{arg}(\dot{\gamma}(t))$ is not monotone. 
%    \item This pair of boundary functions is an example for which condition (c) in Theorem \label{thm:Main} is satisfied but not condition (b):
%$$(f_1(\eta(t)),f_2(\eta(t)))=(\cos(4t)-1,\sin(5t)).$$ In this case $\mathrm{arg}(\dot{\gamma}(t))$ is monotone and $$\abs{\mathrm{Ind}(\dot{\gamma})} = \frac{1}{2},$$ but $$\abs{\mathrm{Ind}(\gamma)}\approx 0.55.$$
%\end{itemize}
%
%
%
%\end{example}


\begin{remark}\label{rem:Discont}
In the setting of theorem \ref{thm:Main}, let $\Gamma=\eta([0,\ell])$ and $\Gamma^d=\eta([0,\ell^d])$ with $\ell^d < \ell$. Boundary functions $f_1,f_2\in C^1(\Gamma)$ that satisfy the assumptions and condition (a) in theorem \ref{thm:Main} can also be used to generate boundary functions $f_1^d, f_2^d \in C^1(\Gamma^d)$ whose zero extensions are discontinuous.  Define $f_i^d$ as
\[
    f_i^d(\eta(t))= f_i(\eta(t)) \chi_{[0,\ell^d]}(t).
\]
This yields solutions $u_i^d$ that satisfy $\mathrm{det} [\nabla u_1^d(x) \, \nabla u_2^d(x)]\neq 0$. This allows for boundary functions that are not captured in condition (b) in theorem \ref{thm:Main}, as in this case it is possible that $1/2<\lvert \mathrm{Ind}(\dot{\gamma^d}) \rvert$, where $\gamma^d(t) = (f_1^d(\eta(t)), f_2^d(\eta(t)))$.
\end{remark}

\beginproof
Assume that one has $\det[\nabla u_1^d(x_0) \, \nabla u_2^d(x_0)]=0$ for some $x_0 \in \Omega$. Then there is a vector $\vec{\alpha} = (\alpha_1, \alpha_2) \in \R^2 \setminus \{0\}$ such that the function 
\[
u^d = \alpha_1 u_1^d + \alpha_2 u_2^d
\]
satisfies $\nabla u^d(x_0) = 0$. 
As $u_i^d \vert_{\partial \Omega}$ is piecewise $C^1$ it follows by the analysis in the proof of theorem \ref{thm:Main} that there exist distinct points $x_1, x_2, x_3, x_4 \in \partial \Omega$ that are in counterclockwise order along $\partial \Omega$ such that
\[
u^d(x_1) > u^d(x_0), \quad u^d(x_2) < u^d(x_0), \quad u^d(x_3) > u^d(x_0), \quad u^d(x_4) < u^d(x_0).
\]
We then consider the function $g^d: [0,\ell] \rightarrow \mathbb{R}$,
\begin{equation*}
    g^d(t) := u^d(\eta(t)) = (\vec{\alpha} \cdot \gamma(t)) \chi_{[0,\ell^d]}(t)
\end{equation*}
where $\gamma(t) = (f_1(\eta(t)), f_2(\eta(t))$ for $t \in [0,\ell]$ as before. We extend $g^d$ by zero to $[0,2\pi)$. Writing $x_j = \eta(t_j)$ where $t_j \in [0,2\pi)$, we have 
\begin{equation} \label{g_contra2}
g^d(t_1) > u^d(x_0), \quad g^d(t_2) < u^d(x_0), \quad g^d(t_3) > u^d(x_0), \quad g^d(t_4) < u^d(x_0).
\end{equation}
Furthermore, we consider the function $g: [0,\ell] \rightarrow \mathbb{R}$ for the same vector $\vec{\alpha}$:
\begin{equation*}
    g(t) := \vec{\alpha} \cdot \gamma(t).
\end{equation*}

Since $\mathrm{\arg}(\dot{\gamma}(t))$ is monotone and $\abs{\mathrm{Ind}(\dot{\gamma})} \leq 1$, it follows that $g'(t)$ has at most two zeros in $(0,\ell)$, or three zeros two of which are at $t=0$ and $t=\ell$. (Again these zeros could be intervals.) Since $u_j|_{\partial \Omega}$ are continuous, we have $f_j(\eta(0)) = f_j(\eta(\ell)) = 0$ and thus  $g(0)=g(\ell)=0$. Suppose that $g'(t)$ has exactly two zeros in $(0,\ell)$. Then since $g'$ must change sign after each zero, there exist two intervals $(0,t_{i})$ and $(t_{i},\ell)$ so that either
\[
g(t) \geq 0 \quad \text{for }t \in (0,t_{i}) \quad \text{and} \quad g(t) \leq 0 \quad \text{for }t \in (t_{i},\ell),
\]
or 
\[
g(t) \leq 0 \quad \text{for }t \in (0,t_{i}) \quad \text{and} \quad g(t) \geq 0 \quad \text{for }t \in (t_{i},\ell).
\]
On the other hand if $g'(t)$ has at most one zero, or three zeros two of which are at $t=0$ and $t=\ell$, then either 
\[
g(t) \geq 0 \quad \text{for } t \in (0,\ell) \quad \text{or} \quad g(t) \leq 0 \quad \text{for } t \in (0,\ell).
\]
The behavior of $g$ translates to $g^d$, as $g^d$ is the restriction of $g$ to the interval $[0,\ell^d]$ with $\ell^d < \ell$. It follows that there are at most two intervals for which $g^d$ is nonnegative and nonpositive respectively, and additionally $(g^d)'$ must change sign after each of its zeros. This is in contradiction with \eqref{g_contra2} as no matter if $u^d(x_0)\geq 0$ or $u^d(x_0) \leq 0$ it is not possible for $g^d$ to have two points for which $g^d(t) \geq u(x_0)$ and two points for which $g^d(t) \leq u(x_0)$ in alternating order.  
\QEDA

\begin{remark}
For boundary functions $f_1$ and $f_2$ that satisfy one of the conditions in theorem \ref{thm:Main} it is determined by the order of the functions whether $\mathrm{det}[\nabla u_1(x) \, \nabla u_2(x)]$ is positive or negative for all $x \in \Omega$.
\end{remark}

\begin{remark} \label{rem:vio}
Let $\Omega$ be a $C^{1,\alpha}$ domain and $f_1,f_2 \in C^{1,\alpha}(\overline{\Omega})$, then $u_i \in C^{1,\alpha}$ on $\overline{\Omega}$ away from the endpoints of $\Gamma$ \cite[Corollary 8.36]{Gilbarg:Trudinger:2001}. Due to the limited view setting $\mathrm{det}[\nabla u_1(x) \, \nabla u_2(x)]$ is zero for $x\in \partial \Omega \setminus \Gamma$. Therefore
\begin{equation*}
    \inf_{x \in \Omega} \mathrm{det}[\nabla u_1(x) \, \nabla u_2(x)] = 0.
\end{equation*}
\end{remark}

\beginproof
We decompose $\nabla u_i$ into two parts with contribution from the unit outward normal $\nu$ and the tangent vector $\omega= \mathcal{J} \nu$ with $\mathcal{J}=\begin{bmatrix} 0 & -1\\ 1 & 0\end{bmatrix}$:
\begin{equation*}
    \nabla u_i = (\nabla u_i \cdot \nu)\nu + (\nabla u_i \cdot \omega)\omega.
\end{equation*}
As $u_i\vert_{\partial \Omega \setminus \Gamma}=0$ by the boundary value problem \eqref{bvpui} it follows that there is no contribution in $\omega$-direction. Therefore both $\nabla u_1\vert_{\partial \Omega \setminus \Gamma}$ and $\nabla u_2\vert_{\partial \Omega \setminus \Gamma}$ are parallel to the unit normal $\nu$ so that $\mathrm{det}[\nabla u_1 \vert_{\partial \Omega \setminus \Gamma} \, \nabla u_2\vert_{\partial \Omega \setminus \Gamma}]=0$. 
\QEDA

\iffalse
\section{Reconstruction procedure}
\label{sec:recProc}
This section lists the reconstruction procedure for an isotropic conductivity $\sigma$ from a $2\times 2$ power density matrix $\mathbf{H}$ based on \cite{monard2012a}. One can extend this procedure for anisotropic conductivities by adding another step following the approach of \cite{BalMonard}. For simplicity, we limit ourselves to the isotropic case. Throughout this section we assume that the boundary functions $f^1$ and $f^2$ were chosen in accordance with theorem \ref{thm:Main} so that the corresponding solutions $u_1$ and $u_2$ entering $\mathbf{H}$ satisfy the non-vanishing Jacobian constraint \eqref{eq:nonvan} and are ordered so that $\text{det}[\nabla u_1 \, \nabla u_2]>0$.\\
\indent The procedure is characterized by two steps. In the first step we reconstruct the angle $\theta$ that enables us to determine the functionals $\mathbf{S}_i=\sqrt{\sigma} \nabla u_i$ from the entries of $H_{ij}=\sigma \nabla u_i \cdot \nabla u_j$. In the second step, we reconstruct $\sigma$ from the functionals $\mathbf{S}_i$.

\subsection{Reconstruction of $\theta$}
We consider the power density matrix $\mathbf{H}$ and the matrix $\mathbf{S}$ composed of the functionals $\mathbf{S}_1$ and $\mathbf{S}_2$: $\mathbf{S}=[\mathbf{S}_1 \, \mathbf{S}_2]$. By definition, $\mathbf{H}$ is symmetric and by the Jacobian constraint and the lower bound on $\sigma$ it follows that $\mathbf{H}$ is positive definite: For any $x=(x_1,x_2)\neq 0, x^T \mathbf{H} x = \sigma \abs{x_1\nabla u_1 + x_2 \nabla u_2}^2>0$ (since $\nabla u_1 $ and $\nabla u_2$ are nonzero and linearly independent by the Jacobian constraint). \\
\indent In order to split the functionals $\mathbf{S}_i$ from the entries of the power density data $H_{ij}$, $\mathbf{S}$ is orthonormalized into a $SO(2)$-valued matrix $\mathbf{R}$: $\mathbf{R}=\mathbf{S}\mathbf{T}^T$. By definition, $\mathbf{R}$ is orthogonal and has determinant one and the transfer matrix $\mathbf{T}$ is determined by the data. The question is, which matrices $\mathbf{T}$ satisfy the equality $\mathbf{R}=\mathbf{S}\mathbf{T}^T$ under the conditions on $\mathbf{R}$. This question has no unique answer, so several choices of $\mathbf{T}$ are possible, for instance $\mathbf{T}=\mathbf{H}^{-\frac{1}{2}}$ or obtaining $\mathbf{T}$ by Gram-Schmidt orthonormalization. As $\mathbf{R}$ is a rotation matrix, it is parameterized by the angle function $\theta$ as follows:
\begin{equation*}
    \mathbf{R}(\theta) = \begin{bmatrix} \cos \theta & -\sin \theta\\ \sin \theta & \cos \theta \end{bmatrix}.
\end{equation*}
From this definition, we see that once $\mathbf{T}$ and $\mathbf{S}$ are known, the function $\theta$ can be computed by
\begin{equation*}
    \theta=\text{arg}(\mathbf{R}_1),
\end{equation*}
where $\mathbf{R}_1$ denotes the first column of $\mathbf{R}$. The orthonormalization technique and thus the choice of $\mathbf{T}$ influences the angle $\theta$. Our choice of $\mathbf{T}$ and the corresponding interpretation of $\theta$ is discussed in subsection \ref{sec:ChoiceTtheta}. \par
Defining $\mathbf{T}=(T_{ij})_{1\leq i,j \leq 2}$ and $\mathbf{T}^{-1}=(T^{ij})_{1\leq i,j \leq 2}$, and letting 
\begin{equation*}
    \mathbf{V_{ij}}=\nabla (T_{i1})T^{1j}+\nabla (T_{i2})T^{2j},
\end{equation*}
then $\theta$ is determined by the following equation \cite[Eq. (65)]{monard2012a}:
\begin{equation}\label{eq:theta}
    \nabla \theta = \mathbf{F},
\end{equation}
with
\begin{equation*}
    \mathbf{F}=\frac{1}{2}(\mathbf{V_{12}}-\mathbf{V_{21}}-\mathcal{J}\nabla \log D),
\end{equation*}
$\mathcal{J}=\begin{bmatrix} 0 & -1\\ 1 & 0\end{bmatrix}$, and $D=(H_{11}H_{22}-H_{12}^2)^{\frac{1}{2}}$. Once $\theta$ is known at at least one point on the boundary one can integrate $\mathbf{F}$ along curves originating from that point to obtain $\theta$ throughout the whole domain. Alternatively, when assuming that $\theta$ is known along the whole boundary one can apply the divergence operator to \eqref{eq:theta} and solve the following Poisson equation with Dirichlet boundary condition:
\begin{equation}\label{eq:thetaBVP}
    \begin{cases}
        \Delta \theta=\nabla \cdot \mathbf{F} & \text{in }\Omega,\\
        \theta=\theta_{\text{true}} & \text{on }\partial \Omega.
    \end{cases}
\end{equation}
In our implementation, we use the second option and discuss in subsection \ref{sec:ChoiceTtheta} knowledge of $\theta$ along the boundary.

\subsection{Reconstruction of $\sigma$}
Reconstruction of $\sigma$ is based on \cite[Eq. (68)]{monard2012a}
\begin{equation}\label{eq:sigmaRec}
    \nabla \log \sigma = \mathbf{G},
\end{equation}
with 
\begin{align*}
    \mathbf{G}&=\cos(2 \theta)\mathbf{K} + \sin(2\theta)\mathbf{K},\\
    \mathbf{K}&=\mathcal{U}(\mathbf{V_{11}}-\mathbf{V_{22}})+\mathcal{J}\mathcal{U}(\mathbf{V_{12}}-\mathbf{V_{21}}) \quad \text{and} \quad \mathcal{U}=\begin{bmatrix} 1 & 0\\ 0 & -1\end{bmatrix}.
\end{align*}
Similarly as for $\theta$ one need to solve a gradient equation to obtain $\sigma$ and has the possibility of either integrating along curves or solving a Poisson equation, assuming knowledge of $\sigma$ in one point or along the whole boundary respectively. We assume knowledge of $\sigma$ along the whole boundary and solve the following Poisson equation with Dirichlet condition:
\begin{equation}\label{eq:sigmaBVP}
    \begin{cases}
        \Delta \log (\sigma)= \nabla \cdot \mathbf{G} &\text{in }\Omega,\\
        \log (\sigma)=\log (\sigma_{\text{true}}) & \text{on }\partial \Omega.
    \end{cases}
\end{equation}

\subsection{Choice of the transfer matrix $\mathbf{T}$ and knowledge of $\theta$}
\label{sec:ChoiceTtheta}

For our implementation, we use Gram-Schmidt orthonormalization to obtain the transfer matrix $\mathbf{T}$:
\begin{equation*}
    \mathbf{T}=\begin{bmatrix} H_{11}^{-\frac{1}{2}} & 0 \\ -H_{12}H_{11}^{-\frac{1}{2}}D^{-1} & H_{11}^{\frac{1}{2}}D^{-1}\end{bmatrix}.
\end{equation*}
By the Jacobian constraint, it follows that $H_{11}>0$ so that $\mathbf{T}$ is well-defined. As a direct consequence of using Gram-Schmidt orthonormalization the first column of $\mathbf{R}$ simplifies to:
\begin{equation*}
    \mathbf{R}_1 = T_{11}\mathbf{S}_1 + T_{12} \mathbf{S}_2 = \frac{\cancel{\sqrt{\sigma}}\nabla u_1}{\cancel{\sqrt{\sigma}}\abs{\nabla u_1}}.
\end{equation*}
Therefore, the angle $\theta$ simply defines the angle between $\nabla u_1$ and the $x_1$-axis. Hence,
\begin{equation}\label{eq:thetau1}
    \theta = \text{arg}(\nabla u_1).
\end{equation}
In addition, following this definition for $\mathbf{T}$ the vector fields $\mathbf{V_{ij}}$ can be written explicitly in terms of $\mathbf{H}$:
\begin{align}\label{eq:Vexp}
\begin{aligned}
    \mathbf{V_{11}}&= \nabla \log H_{11}^{-\frac{1}{2}}, & \mathbf{V_{12}}&=0,\\ \mathbf{V_{21}}&= -\frac{H_{11}}{D} \nabla \left( \frac{H_{12}}{H_{11}}\right), & \mathbf{V_{22}}&=\nabla \log \left( \frac{H_{11}^{\frac{1}{2}}}{D}\right).
    \end{aligned}
\end{align}
Knowledge of $\theta$ at the boundary is essential for the reconstruction procedure. By this definition of $\mathbf{T}$, knowledge of $\theta$ is directly related to knowledge of the gradient $\nabla u_1$ and the current $\sigma \nabla u_1$, as both vector fields have the same direction. We decompose $\sigma \nabla u_1$ into two parts with contribution from the unit outward normal $\nu$ and the tangent vector $\omega=\mathcal{J}\nu$:
\begin{equation*}
    \sigma \nabla u_1 = (\sigma \nabla u_1 \cdot \nu)\nu + (\sigma \nabla u_1 \cdot \omega)\omega.
\end{equation*}
As along the whole boundary $u_1$ and $\sigma$ are known, the contribution from $\sigma \nabla u_1 \cdot \omega$ is known as well. Furthermore, along the part of the boundary $\partial \Omega \backslash \Gamma$ we have additional information as $u_1$ vanishes. Therefore, the only contribution is from the unit outward normal $\nu$, so that on this part of the boundary $\sigma \nabla u_1$ has either the direction of $\nu$, $-\nu$ or the zero vector. However, in order to have full information of $\theta$ along the boundary one needs knowledge about the Neumann data $\sigma \nabla u_1 \cdot \nu$.

\fi

\section{Numerical Examples}

\begin{equation}\label{logsym}
    \log_{\mathrm{sym}}(x) = \mathrm{sign}(x) \log \lp 1+\abs{\frac{x}{C}} \rp
\end{equation}
we use $C=10^{-3}$. This formula is based on \cite[eq.(4)]{webber2013a}.

\iffalse

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/AdaptH11}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/AdaptH12}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/AdaptH22}
        %\caption*{10\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/CoordH11}
        \caption*{$\log(H_{11})$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/CoordH12}
        \caption*{$\log_{\mathrm{sym}}(H_{12})$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/CoordH22}
        \caption*{$\log(H_{22})$}
    \end{minipage}
    \caption{Log plots of the power densities in case of adapted boundary functions (upper row) and cut off boundary functions (lower row). As $H_{12}$ holds both positive and negative values we use the bi-symmetric transformation $\log_{\mathrm{sym}}$ in \eqref{logsym}.}
    \label{fig:sigmaRecs}
\end{figure}

\fi

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures2/PlaceholderHijs2.png}
    \caption{Log plots of the power densities in case of adapted boundary functions (upper row) and cut off boundary functions (lower row). As $H_{12}$ holds both positive and negative values we use the bi-symmetric transformation $\log_{\mathrm{sym}}$ in \eqref{logsym}.}
    \label{fig:enter-label}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetFull.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetHuge.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetLar.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetMedLar.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetMed.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetSmaMed.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetSma.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logDetMini.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \caption{Log dets adapted.}
    \label{fig:sigmaRecs}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logH11Full.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logH11Huge.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logH11Lar.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logH11MedLar.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/LogH11Med.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/LogH11SmaMed.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logH11Sma.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/logH11Mini.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \caption{Log H11s adapted.}
    \label{fig:sigmaRecs}
\end{figure}



\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{Figures2/TrueSigma.pdf}
    \caption{True phantom.}
    \label{fig:enter-label}
\end{figure}


\iffalse
\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptFull}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptHuge}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptLar}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptMedLar}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptMed}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptSmaMed}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptSma}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptMini}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs}
\end{figure}
\fi

\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures2/PlaceholderRecs.png}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:enter-label}
\end{figure}





\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{CoordNoise/TrueSigma.pdf}
    \caption{Caption}
    \label{fig:enter-label}
\end{figure}

%\begin{figure}[ht!]
%    \centering
%        \includegraphics[width=\linewidth]{Figures2/Noisefig.png}
%    \caption{Reconstructions for varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
%    \label{fig:sigmaRecs}
%\end{figure}

\iffalse

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Adapt1noise}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Adapt5noise}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Adapt10noise}
        %\caption*{10\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Coord1noise}
        \caption*{$1\%$ noise, $\lambda_{\min}=10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Coord5noise}
        \caption*{$5\%$ noise, $\lambda_{\min}=10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Coord10noise}
        \caption*{$10\%$ noise, $\lambda_{\min}=10^{-6}$}
    \end{minipage}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs}
\end{figure}

\fi


\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures2/PlaceholderNoise2.png}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:enter-label}
\end{figure}


\iffalse
\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptFull}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Huge}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Lar}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/MedLar}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Med}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/SmaMed}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Sma}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Mini}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs}
\end{figure}
\fi

%\begin{figure}
%    \centering
%    \includegraphics[width=\textwidth,trim={2.6cm 1.1cm 4cm 1.1cm},clip]{AdaptedNoise/ContMedNoise11e7.pdf}
%    \caption{Caption}
%    \label{fig:enter-label}
%\end{figure}


\clearpage

\iffalse

\section{Conclusions}
In this work, we have derived sufficient conditions on two boundary functions so that the corresponding solutions to the conductivity equation satisfy a non-vanishing Jacobian constraint in limited view. This approach allows for boundary functions that have discontinuities. This is relevant for Acousto-Electric Tomography and Current Density Imaging both in limited view and in full view settings, as the conditions and thus the use of discontinuous boundary functions apply for both settings. \par
We illustrated how these conditions could be used for numerical examples of reconstructing the conductivity from power density data in limited view following the approach of \cite{monard2012a}. It was evident from the numerical examples how the non-vanishing Jacobian constraint was almost violated close to the boundary that could not be controlled. This follows from the zero Dirichlet condition on this part of the boundary: Here the two corresponding solutions have both the direction of the unit normal so that the non-vanishing Jacobian constraint cannot be satisfied on this part of the boundary. Nevertheless, without noise it was possible to obtain decent reconstructions of the conductivity when the support of the boundary of control was at least half the size of the full boundary. For smaller boundaries of control the numerical results get unreliable due to small values of the Jacobian. Therefore in general it is almost impossible to add even small levels of noise while maintaining positive definiteness of the measurement matrix. To account for this, we used a small positive lower bound for the eigenvalues of the measurement matrix. This worked well in the numerical experiments even for high noise levels. However, in this approach especially values close to the part of the boundary that cannot be controlled are affected by the lower bound. When the lower bound is high this might be in contradiction with the assumption that values should be small in this region. This is especially a problem when using discontinuous boundary conditions as the lower bound needs to be chosen large when the noise level is high. \par
We mention that the proposed conditions in order to obtain solutions satisfying the non-vanishing Jacobian constraint are not optimal. Especially for the case of discontinuous boundary functions there is a possibility that \ref{thm:Main} (b) can be relaxed, as we are aware of functions that are more general than allowed here as indicated in Remark \ref{rem:Discont}.


\paragraph*{Acknowledgements}
The authors would like to express their sincere gratitude to our Nuutti Hyv\"onen for suggesting how to solve the boundary value problem \eqref{bvpui} numerically with discontinuous boundary conditions, and for providing the \matlab{} code to solve the boundary value problem \eqref{eq:LapBVP} semi-analytically as discussed in section \ref{sec:DBC}. M.S.\ was partly supported by the Academy of Finland (Centre of Excellence in Inverse Modelling and Imaging, grant 284715) and by the European Research Council under Horizon 2020 (ERC CoG 770924).
\fi

==> Text2.tex <==
%To dos:
%Fix equation (13)
%Remember to put the real figures in again
%Report the relative error for the reconstruction
%Acknowledgements section
%Fix mathbf notation
%Remark that this also holds for anisotropic conductivities
%Show relative error for both adapted and coordinate functions

\section{Introduction}
In 1980 A.P.Calderón proposed the inverse problem whether it is possible to recover the electrical conductivity by making voltage and current measurements at the boundary. This approach has been realized in medical imaging by the modality \textit{electrical impedance tomography (EIT)}. However, the EIT problem is severely ill-posed and the corresponding reconstructions have low resolution. In order to address these issues, hybrid inverse problems were introduced. For these kind of inverse problems the reconstruction procedure typically consists of two steps: First combine two imaging modalities so that interior measurements can be obtained; secondly recover the conductivity from these interior measurements. We focus on applications that combine the EIT approach with magnetic resonance imaging (MRI) or acoustic waves. The former approaches are known as current density imaging (CDI) \cite{WidlakScherzer, Bal2013_survey, LiSchotlandYangZhong} and Magnetic Resonance Electric Impedance Tomography (MREIT) \cite{Seo_2005,SeoWoo11} and the latter approach is known as Acousto-Electric Tomography (AET) \cite{Zhang:Wang:2004, ammari2008a}. While the EIT approach yields high contrast of the reconstruction, the MRI and acoustic waves yield high resolution of the reconstruction.\\

The mathematical framework behind these applications is the conductivity equation that links the electric potential $u$ with the electrical conductivity $\sigma \in L^{\infty}(\Omega)$:
\begin{equation}\label{condeq}
    \begin{cases}
    -\mathrm{div}(\sigma \nabla u_i)=0 & \text{in }\Omega,\\
    \sigma \nabla u_i \cdot \nu = g_i & \text{on }\partial \Omega,
\end{cases}
\end{equation}
here $\Omega \subseteq \R^2$ models a two-dimensional medium with Lipschitz boundary $\partial \Omega$, $\nu$ is the outward unit normal and the unique solutions $u_i \in H^1(\Omega)$ correspond to different potentials $g_i \in H^{-\frac{1}{2}}(\partial \Omega)$ with $\int_{\partial \Omega} g_i \,\mathrm{d}S=0$ imposed on $\partial \Omega$. 
%The EIT procedure corresponds to recovering $\sigma$ from the potential to current map $$\Lambda_g : g \mapsto \sigma \nabla u \cdot \nu \vert_{\partial \Omega}.$$
The interior measurements for CDI and MREIT are current densities $\sigma \nabla u_i$ corresponding to two different potentials $g_1$ and $g_2$ imposed. For AET the interior measurements are power densities $\mathbf{H}_{ij}=\sigma \nabla u_i \cdot \nabla u_j$ also corresponding to two different potentials $g_1$ and $g_2$ imposed. The inverse problem of recovering the conductivity from $\sigma \nabla u_i$ or $\sigma \nabla u_i \cdot \nabla u_j$ requires inversions of the matrix $[\nabla u_1 \, \, \nabla u_2]$. So in order for the reconstruction procedure to be well-defined one requires that the following \textit{Jacobian} is non-vanishing:
\begin{equation} \label{eq:nonvan}
    \det [\nabla u_1(x) \, \, \nabla u_2(x)] \neq 0, \quad x \in \Omega.
\end{equation}
The question of how to choose boundary conditions in order to have no vanishing Jacobian has been mainly addressed for Dirichlet boundary conditions. This dates back to Radó, Kneser and Choquet in 1926 and 1945 and is formulated in the Radó-Kneser-Choquet theorem \cite{Rado26,Kneser26,Choquet45}. Here they studied the non-constant coefficient case $\sigma=1$. This result has been generalized to non-constant coefficients and anisotropic conductivities in \cite{Alessandrini86,Alessandrini87,AlessandriniMagnanini94,AlessandriniNesi01,BaumanMariniNesi01,alessandriniNesi15}. For instance, \cite{BaumanMariniNesi01} require that $g=(g_1,g_2)$ is a $C^1$ diffeomorphism and maps $\partial \Omega$ onto the boundary of a convex domain for the condition \eqref{eq:nonvan} to hold. A discussion of such results for Dirichlet boundary conditions is given in \cite{AlbertiCapdeboscq18}. Recent work addresses random boundary functions and the probability for satisfying constraints on the form \eqref{eq:nonvan} \cite{AlbertiArxiv}. \\

We consider a limited view setting, where we only have access to some non-empty closed part of the boundary $\Gamma \subseteq \partial \Omega$ and on the remaining boundary $\sigma \nabla u_i \cdot \nu$ is vanishing:
\begin{equation}\label{condeqlim}
    \begin{cases}
    -\mathrm{div}(\sigma \nabla u_i)=0 & \text{in }\Omega,\\
    \sigma \nabla u_i \cdot \nu = f_i & \text{on }\Gamma,\\
    \sigma \nabla u_i \cdot \nu = 0 & \text{on }\partial \Omega \setminus \Gamma,\\
\end{cases}
\end{equation}
with $f_i \in C(\Gamma)$ and $\int_{\Gamma} f_i \,\mathrm{d}S=0$ so that $\sigma \nabla u_i \vert_{\partial \Omega} \in H^{-\frac{1}{2}}(\partial \Omega)$ and $u_i \in H^1(\Omega)$. The question of choosing boundary functions $f_1$ and $f_2$ for a non-vanishing Jacobian has been addressed for this limited view setting in \cite{Salo2022} (Dirichlet boundary conditions) and \cite{Jensen2023} (Mixed Dirichlet and Neumann boundary conditions). We establish similar results for this limited 
view setting by extending the result in \cite[Theorem 2.8]{AlessandriniMagnanini94} from no critical points to a non-vanishing Jacobian. We give explicit conditions on the boundary functions $f_1$ and $f_2$ in terms of the winding number associated to the curve generated by $f_1$ and $f_2$ (as this not necessarily yields a closed curve we consider a generalized definition). We test such boundary functions in practice by reconstructing $\sigma$ numerically from the corresponding power density data $\mathbf{H}_{ij}=\sigma \nabla u_i \cdot \nabla u_j$ in limited view following the approach of Acousto-electric tomography.\\

Section 2 lists the main result of explicit conditions on the boundary functions $f_1$ and $f_2$. Section 3 lists an analytic reconstruction procedure of $\sigma$ from $\mathbf{H}\in \R^{2\times 2}$ based on \cite{BalMonard}. In section 4 we test boundary functions chosen in accordance with the main result for reconstruction of $\sigma$ from $\mathbf{H}\in \R^{2\times 2}$. We conclude by a discussion in section 5.
 





\section{Main results}

We state the following proposition without proof corresponding to \cite[Thm 2.8]{AlessandriniMagnanini94}.
\begin{proposition}\label{prop:am94}
    Let $\Omega \subset \R^2$ be a simply connected bounded Lipschitz domain and let $\sigma \in L^{\infty}(\Omega)$ satisfy $\lambda \leq \sigma$ for some $\lambda \in (0,1)$. Let $g \in H^{-\frac{1}{2}}(\partial \Omega)$ with $\int_{\partial \Omega} g \, \mathrm{d}S=0$ and $u \in H^1(\Omega)$ be a nonconstant solution of 
\begin{equation*}
\begin{cases}
    -\mathrm{div}(\sigma \nabla u)=0 & \text{in }\Omega,\\
    \sigma \nabla u \cdot \nu = g & \text{on }\partial \Omega.
\end{cases}
\end{equation*}
Denote by $2M$ the number of closed arcs $\Gamma_1,...,\Gamma_{2M}$ into which $\partial \Omega$ can be split for which $(-1)^j g\geq 0$ on $\Gamma_j$, $j=1,...,2M$. Then the number of interior critical points $N$ satisfies:
\begin{equation*}
    N \leq M - 1.
 \end{equation*}
\end{proposition}

The following lemma is a consequence of Proposition \ref{prop:am94}:

\begin{lemma}\label{lem:4points}
    Let $\Omega, \sigma, u$ and $g$ be as in proposition \ref{prop:am94}. By the proposition it follows that when $\Omega$ has one critical point $x_0 \in \Omega$ so that $\nabla u(x_0)=0$ then $\partial \Omega$ must be composed of at least 4 closed arcs $\Gamma_1, \Gamma_2, \Gamma_3, \Gamma_4$ for which $(-1)^j g \geq 0$. Hence, there must exist points $x_1 \in \Gamma_1, x_2 \in \Gamma_2, x_3 \in \Gamma_3$ and $x_4 \in \Gamma_4$ such that
    \[
\sigma \nabla u \cdot \nu \vert_{x=x_1} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_2} > 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_3} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_4} > 0.\]
\end{lemma}

We want to revisit the concept of the winding number of a continuous curve $\gamma: [0,\ell] \to \R^2$ and generalize this to the setting were $\gamma$ is not closed, i.e $\gamma(0) \neq \gamma(\ell)$. We assume that $\gamma(t) \neq 0$ for all $t \in [0,\ell]$. We then rewrite $\gamma(t)$ in terms of polar coordinates as 
\[
\gamma(t) = r(t) e^{i\phi(t)}
\]
where $r(t) = \abs{\gamma(t)}$ and $\phi(t)$ are continuous functions in $[0,\ell]$. The angle function 
\[
\mathrm{arg}(\gamma(t)) := \phi(t)
\]
is well defined modulo a constant in $2\pi \mathbb{Z}$. We define 
\[
\mathrm{Ind}(\gamma) := \frac{\mathrm{arg}(\gamma(\ell)) - \mathrm{arg}(\gamma(0))}{2\pi}.
\]
If $\gamma$ is closed, i.e.\ $\gamma(0) = \gamma(\ell)$, then $\mathrm{Ind}(\gamma)$ is the winding number of the curve $\gamma(t)$, which is an integer. If $\gamma$ is not closed but $\mathrm{arg}(\gamma(t))$ is monotone (i.e.\ nondecreasing or nonincreasing), we may still interpret $\mathrm{Ind}(\gamma)$ as the winding number of $\gamma(t)$, and this is then a real number.

We now give a sufficient conditions on a pair of boundary data vanishing outside an arc $\Gamma$ such that the corresponding solutions $u_1, u_2$ satisfy $\mathrm{det} [\nabla u_1(x) \, \nabla u_2(x)]\neq 0$ everywhere in $\Omega$. Note that this can be seen as a consequence of \cite[Theorem 2.8]{AlessandriniMagnanini94}.

\begin{theorem}\label{thm:Main}
Let $\Omega \subset \R^2$ be a bounded simply connected Lipschitz domain with continuous boundary curve $\eta: [0,2\pi] \to \partial \Omega$, and let $\sigma \in L^{\infty}(\Omega)$ satisfy $\lambda \leq \sigma$ for some $\lambda \in (0,1)$. Let $\Gamma = \eta([0,\ell])$ be a closed arc in $\partial \Omega$. Let $f_1, f_2 \in C(\Gamma)$ be linearly independent so that $\int_{\Gamma} f_1 \,\mathrm{d}S=\int_{\Gamma} f_2 \,\mathrm{d}S=0$‚ and assume that $u_i$ is the unique solution of 
\begin{equation}\label{bvpui}
    \begin{cases}
        -\mathrm{div}(\sigma \nabla u_i)=0 & \text{in }\Omega,\\
        \sigma \nabla u_i \cdot \nu=f_i & \text{on }\Gamma ,\\
        \sigma \nabla u_i \cdot \nu = 0 & \text{on }\partial \Omega \backslash \Gamma.
    \end{cases}
\end{equation}
Assume that the curve $\gamma: [0,\ell] \to \R^2$ defined by $\gamma(t) = (f_1(\eta(t)), f_2(\eta(t)))$ satisfies $\gamma(t) \neq 0$ for all $t \in [0,\ell]$, $\mathrm{arg}(\gamma(t))$ is monotone, and $$\abs{\mathrm{Ind}(\gamma)} \leq 1.$$
Then $\mathrm{det} [\nabla u_1(x) \, \nabla u_2(x)]\neq 0$ for all $x \in \Omega$.

\end{theorem}

%\begin{theorem}\label{thm:Main}
%Let $\Omega \subset \R^2$ be a bounded simply connected domain with $C^1$ boundary curve $\eta: [0,2\pi] \to \partial \Omega$, and let $\sigma \in C^{0,\alpha}(\overline{\Omega};\R^{2\times 2})$ satisfy \eqref{ellip}. Let $\Gamma = \eta([0,\ell])$ be a closed arc in $\partial \Omega$. Let $f_1, f_2 \in C^1(\Gamma)$ be linearly independent‚ and assume that $u_i$ is the unique solution of 
%\begin{equation}\label{bvpui}
%    \begin{cases}
%        -\mathrm{div}(\sigma \nabla u_i)=0 & \text{in }\Omega,\\
%        \sigma \nabla u_i \cdot \nu=f_i & \text{on }\Gamma ,\\
%        \sigma \nabla u_i \cdot \nu = 0 & \text{on }\partial \Omega \backslash \Gamma.
%    \end{cases}
%\end{equation}
%Assume that the curve $\gamma: [0,\ell] \to \R^2$, $\gamma(t) = (f_1(\eta(t)), f_2(\eta(t)))$ is regular,  and that one of the following holds:
%\begin{enumerate}
%    \item[(a)] $\sigma \nabla u_i \cdot \nu\vert_{\partial \Omega}$ are continuous, and $\mathrm{arg}(\gamma(t))$ is monotone, and $\abs{\mathrm{Ind}(\gamma)} \leq 1$; or 
%    \item[(b)] $\sigma \nabla u_i \cdot \nu\vert_{\partial \Omega}$ are continuous at $\eta(0)$, and $\mathrm{arg}(\gamma(t))$ is monotone, and $\abs{\mathrm{Ind}(\gamma)} \leq 1/2$; or
%    \item[(c)] $\sigma \nabla u_i \cdot \nu\vert_{\partial \Omega}$ are continuous at $\eta(0)$, and $\mathrm{arg}(\dot{\gamma(t)})$ is monotone, and $\abs{\mathrm{Ind}(\dot{\gamma})} \leq 1/2$.
%\end{enumerate}
%Then $\mathrm{det} [\nabla u_1(x) \, \nabla u_2(x)]\neq 0$ for all $x \in \Omega$.
%
%\end{theorem}
\beginproof
Assume that the result holds, but one has $\mathrm{det} [\nabla u_1(x_0) \, \nabla u_2(x_0)] =  0$ for some $x_0 \in \Omega$. Then there is a vector $\vec{\alpha} = (\alpha_1, \alpha_2) \in \R^2 \setminus \{0\}$ such that the function 
\[
u = \alpha_1 u_1 + \alpha_2 u_2
\]
satisfies $\nabla u(x_0) = 0$. Note that if $u$ is a constant, then 
\begin{equation*}
    0=\sigma \nabla u \cdot \nu\vert_{\Gamma} = \alpha_1 \sigma \nabla u_1 \cdot \nu\vert_{\Gamma} + \alpha_2 \sigma \nabla u_2 \cdot \nu\vert_{\Gamma} = \alpha_1 f_1 + \alpha_2 f_2 
\end{equation*}
Hence $f_1$ and $f_2$ would be linearly dependent. Thus, we may assume that $u$ is nonconstant. Note that $\sigma \nabla u_i|_{\partial \Omega} \cdot \nu$ are discontinuous, but piecewise continuous and hence they are in $H^{-\frac{1}{2}}(\partial \Omega)$. Then by Lemma \ref{lem:4points} there exist distinct points $x_1, x_2, x_3, x_4 \in \partial \Omega$ that are in counterclockwise order along $\partial \Omega$ such that 
\[
\sigma \nabla u \cdot \nu \vert_{x=x_1} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_2} > 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_3} < 0, \quad \sigma \nabla u \cdot \nu \vert_{x=x_4} > 0.\]
Consider the function $h: [0,\ell] \to \R$ given by 
\begin{equation}\label{g_fun}
h(t) := \sigma(\eta(t)) \nabla u(\eta(t)) \cdot \nu(\eta(t))= \vec{\alpha} \cdot \gamma(t).
\end{equation}
Extend $h$ by zero to $[0,2\pi)$. Writing $x_j = \eta(t_j)$ where $t_j \in [0,2\pi)$, we have 
\begin{equation} \label{g_contra}
h(t_1) > 0, \quad h(t_2) < 0, \quad h(t_3) > 0, \quad h(t_4) < 0.
\end{equation}
We may assume that $t_1 < t_2 < t_3 < t_4$ (possibly after a cyclic permutation of the indices and after changing $h$ to $-h$).

We now assume that the result holds, and want to derive a contradiction with \eqref{g_contra}. Since $\gamma(t)\neq 0$, $\mathrm{arg}(\gamma(t))$ is monotone and $\abs{\mathrm{Ind}(\gamma(t))} \leq 1$, it follows that $h(t)$ either has at most two zeros in $[0,\ell]$, or has three zeros two of which are at $t=0$ and $t=\ell$. Note that if the argument is not strictly monotone, we make the interpretation that some of these zeros of $h$ could be intervals. Since we assume that $f_1,f_2\in C(\Gamma)$ it follows that $h \in C(\Gamma)$. Now by \eqref{g_contra} $h$ has a zero in the interval $(t_1,t_2)$, a zero in the interval $(t_2,t_3)$ and a zero in the interval $(t_3,t_4)$. Therefore $h$ has at least three zeros in $(0,\ell)$. This is a contradiction. 
\QEDA


\begin{remark}\label{rem:corrdcut}
    Let $\Omega$ be a convex domain and denote by $(f_1^\ell,f_2^\ell)$ normalized cut offs of the coordinate functions $(f_1,f_2)=(x_1,x_2)$. Let $\Gamma = \eta([0,\ell])$ be the support of $f_i^\ell$ and $\partial \Omega = \eta([0,2\pi])$ be the support of $f_i$ with $\ell < 2\pi$. These normalized cut offs are defined by:
    \begin{equation*}
        f_i^\ell(\eta(t)) = f_i(\eta(t)) \chi_{[0,\ell]}(t) - \frac{\int_{\partial \Omega} f_i(\eta(t)) \chi_{[0,\ell]}(t)\,\mathrm{d}t}{\ell}.
    \end{equation*}
    They are automatically captured by Theorem \ref{thm:Main} as $\int_\Gamma f_i^\ell \, \mathrm{d}t=0$ and $\abs{\mathrm{Ind}(f_1(\eta(t)),f_2(\eta(t)))}=1$ so that $\abs{\mathrm{Ind}(f_1^\ell(\eta(t)),f_2^\ell(\eta(t)))}<1$.
\end{remark}






\begin{remark}
For boundary functions $f_1$ and $f_2$ that satisfy one of the conditions in theorem \ref{thm:Main} it is determined by the order of the functions whether $\mathrm{det}[\nabla u_1(x) \, \nabla u_2(x)]$ is positive or negative for all $x \in \Omega$.
\end{remark}

\begin{remark} \label{rem:vio}
Let $\Omega$ be a $C^{1,\alpha}$ domain and $f_1,f_2 \in C^{1,\alpha}(\overline{\Omega})$, then $u_i \in C^{1,\alpha}$ on $\overline{\Omega}$ away from the endpoints of $\Gamma$ \cite[Corollary 8.36]{Gilbarg:Trudinger:2001}. Due to the limited view setting $\mathrm{det}[\nabla u_1(x) \, \nabla u_2(x)]$ is zero for $x\in \partial \Omega \setminus \Gamma$. Therefore
\begin{equation*}
    \inf_{x \in \Omega} \mathrm{det}[\nabla u_1(x) \, \nabla u_2(x)] = 0.
\end{equation*}
\end{remark}

\beginproof
We decompose $\nabla u_i$ into two parts with contribution from the unit outward normal $\nu$ and the unit tangent vector $\omega= \mathcal{J} \nu$ with $\mathcal{J}=\begin{bmatrix} 0 & -1\\ 1 & 0\end{bmatrix}$:
\begin{equation*}
    \nabla u_i = (\nabla u_i \cdot \nu)\nu + (\nabla u_i \cdot \omega)\omega.
\end{equation*}
As $\sigma \nabla u_i \cdot \nu \vert_{\partial \Omega \setminus \Gamma}=0$ by the boundary value problem \eqref{bvpui} it follows that there is no contribution in $\nu$-direction. Therefore both $\nabla u_1\vert_{\partial \Omega \setminus \Gamma}$ and $\nabla u_2\vert_{\partial \Omega \setminus \Gamma}$ are parallel to the unit tangent vector $\omega$ so that $\mathrm{det}[\nabla u_1 \vert_{\partial \Omega \setminus \Gamma} \, \nabla u_2\vert_{\partial \Omega \setminus \Gamma}]=0$. 
\QEDA

\section{Reconstruction procedure}
\label{sec:recproc}
This section lists the analytic reconstruction procedure of an isotropic conductivity $\sigma$ from interior power density measurements $H_{ij}=\sigma \nabla u_i \cdot \nabla u_j$ corresponding two different boundary functions $f_1$ and $f_2$ imposed. This approach is fully based on \cite{monard2012a}. We only list the main equations and refer the reader to \cite{monard2012a} for more details.\\

The reconstruction procedure is split into two steps: Step one to split the functionals $S_i=\sqrt{\sigma} \nabla u_i$ apart and the second step to recover $\sigma$ from $S_i=\sqrt{\sigma} \nabla u_i$ for $i=1,2$. 

\subsection{Reconstruction of $S_i=\sqrt{\sigma} \nabla u_i$}
Reconstructing $S_i=\sqrt{\sigma} \nabla u_i$ is realized by orthonormalizing the matrix $S=[S_1 \, \, S_2]$ into an $SO(2)$-valued matrix $R$: $R = S T^T$. The matrix $R$ is a rotation matrix that is orthogonal and has determinant one and $T$ is a matrix only depending on the data. $R$ can be parameterized by an angle function $\theta$:
\begin{equation*}
    R(\theta) = \begin{bmatrix} \cos \theta & -\sin \theta\\ \sin \theta & \cos \theta \end{bmatrix}.
\end{equation*}
We introduce the functions $V_{ij}$ that depend on entries of $T$ and derivatives of its entries:
\begin{equation*}
    V_{ij}=\nabla (T_{i1})T^{1j}+\nabla (T_{i2})T^{2j}, \quad i,j=1,2
\end{equation*}
here $T^{ij}$ denotes entries in $T^{-1}$. The first step in the reconstruction procedure then consists of reconstructing $\theta$ and thus $S$ from the following equation \cite[Eq. (65)]{monard2012a}:
\begin{equation}\label{eq:theta}
    \nabla \theta = \mathbf{F},
\end{equation}
with
\begin{equation*}
    \mathbf{F}=\frac{1}{2}(\mathbf{V_{12}}-\mathbf{V_{21}}-\mathcal{J}\nabla \log D),
\end{equation*}
where $\mathcal{J}=\begin{bmatrix} 0 & -1\\ 1 & 0\end{bmatrix}$, and $D=(H_{11}H_{22}-H_{12}^2)^{\frac{1}{2}}$.  Once $\theta$ is known at at least one point on the boundary one can integrate $\mathbf{F}$ along curves originating from that point to obtain $\theta$ throughout the whole domain. If one assumes that $\theta$ is known along the whole boundary one can apply the divergence operator to \eqref{eq:theta} and solve the following Poisson equation with Dirichlet boundary condition:
\begin{equation}\label{eq:thetaBVP}
    \begin{cases}
        \Delta \theta=\nabla \cdot \mathbf{F} & \text{in }\Omega,\\
        \theta=\theta_{\text{true}} & \text{on }\partial \Omega.
    \end{cases}
\end{equation}

\begin{remark}
For implementation we use Gram-Schmidt orthonormalization to obtain the transfer matrix $\mathbf{T}$:
    \begin{equation*}
    \mathbf{T}=\begin{bmatrix} H_{11}^{-\frac{1}{2}} & 0 \\ -H_{12}H_{11}^{-\frac{1}{2}}D^{-1} & H_{11}^{\frac{1}{2}}D^{-1}\end{bmatrix}.
\end{equation*}
This implies that the angle $\theta$ has the interpretation:
\begin{equation*}
    \theta=\text{arg}(\mathbf{R}_1)=\frac{\nabla u_1}{\abs{\nabla u_1}},
\end{equation*}
where $\mathbf{R}_1$ is the first column of $\mathbf{R}$. This implies that $\theta$ describes the angle between $\nabla u_1$ and the $x_1$-axis.
\end{remark}

\subsection{Reconstruction of $\sigma$}
Reconstruction of $\sigma$ is based on \cite[Eq. (68)]{monard2012a}
\begin{equation}\label{eq:sigmaRec}
    \nabla \log \sigma = \mathbf{G},
\end{equation}
with 
\begin{align*}
    \mathbf{G}&=\cos(2 \theta)\mathbf{K} + \sin(2\theta)\mathbf{K},\\
    \mathbf{K}&=\mathcal{U}(\mathbf{V_{11}}-\mathbf{V_{22}})+\mathcal{J}\mathcal{U}(\mathbf{V_{12}}-\mathbf{V_{21}}) \quad \text{and} \quad \mathcal{U}=\begin{bmatrix} 1 & 0\\ 0 & -1\end{bmatrix}.
\end{align*}
Similarly to reconstruction of $\theta$ one can solve this gradient equation by integrating along curves if $\sigma$ is known at one point at the boundary or solving the following boundary value problem if $\sigma$ is assumed known along the whole boundary:
\begin{equation}\label{eq:sigmaBVP}
    \begin{cases}
        \Delta \log (\sigma)= \nabla \cdot \mathbf{G} &\text{in }\Omega,\\
        \log (\sigma)=\log (\sigma_{\text{true}}) & \text{on }\partial \Omega.
    \end{cases}
\end{equation}

\begin{remark}
    For implementation we assume that $\theta$ and $\sigma$ are known along the whole boundary and reconstruct these functions by solving the boundary value problems \eqref{eq:thetaBVP} and \eqref{eq:sigmaBVP}. This requires knowledge of $\theta$ and $\sigma$ at the boundary. Information about the former requires information about $\sigma$ and $u_1$ at the boundary, since these yield information about the tangential component of $\sigma \nabla u_1$. Combining this information with knowledge of $\sigma \nabla u_1 \cdot \nu$ yields information about $\sigma \nabla u_1$ and thus $\theta$. 
\end{remark}



\iffalse
\section{Reconstruction procedure}
\label{sec:recProc}
This section lists the reconstruction procedure for an isotropic conductivity $\sigma$ from a $2\times 2$ power density matrix $\mathbf{H}$ based on \cite{monard2012a}. One can extend this procedure for anisotropic conductivities by adding another step following the approach of \cite{BalMonard}. For simplicity, we limit ourselves to the isotropic case. Throughout this section we assume that the boundary functions $f^1$ and $f^2$ were chosen in accordance with theorem \ref{thm:Main} so that the corresponding solutions $u_1$ and $u_2$ entering $\mathbf{H}$ satisfy the non-vanishing Jacobian constraint \eqref{eq:nonvan} and are ordered so that $\text{det}[\nabla u_1 \, \nabla u_2]>0$.\\
\indent The procedure is characterized by two steps. In the first step we reconstruct the angle $\theta$ that enables us to determine the functionals $\mathbf{S}_i=\sqrt{\sigma} \nabla u_i$ from the entries of $H_{ij}=\sigma \nabla u_i \cdot \nabla u_j$. In the second step, we reconstruct $\sigma$ from the functionals $\mathbf{S}_i$.

\subsection{Reconstruction of $\theta$}
We consider the power density matrix $\mathbf{H}$ and the matrix $\mathbf{S}$ composed of the functionals $\mathbf{S}_1$ and $\mathbf{S}_2$: $\mathbf{S}=[\mathbf{S}_1 \, \mathbf{S}_2]$. By definition, $\mathbf{H}$ is symmetric and by the Jacobian constraint and the lower bound on $\sigma$ it follows that $\mathbf{H}$ is positive definite: For any $x=(x_1,x_2)\neq 0, x^T \mathbf{H} x = \sigma \abs{x_1\nabla u_1 + x_2 \nabla u_2}^2>0$ (since $\nabla u_1 $ and $\nabla u_2$ are nonzero and linearly independent by the Jacobian constraint). \\
\indent In order to split the functionals $\mathbf{S}_i$ from the entries of the power density data $H_{ij}$, $\mathbf{S}$ is orthonormalized into a $SO(2)$-valued matrix $\mathbf{R}$: $\mathbf{R}=\mathbf{S}\mathbf{T}^T$. By definition, $\mathbf{R}$ is orthogonal and has determinant one and the transfer matrix $\mathbf{T}$ is determined by the data. The question is, which matrices $\mathbf{T}$ satisfy the equality $\mathbf{R}=\mathbf{S}\mathbf{T}^T$ under the conditions on $\mathbf{R}$. This question has no unique answer, so several choices of $\mathbf{T}$ are possible, for instance $\mathbf{T}=\mathbf{H}^{-\frac{1}{2}}$ or obtaining $\mathbf{T}$ by Gram-Schmidt orthonormalization. As $\mathbf{R}$ is a rotation matrix, it is parameterized by the angle function $\theta$ as follows:
\begin{equation*}
    \mathbf{R}(\theta) = \begin{bmatrix} \cos \theta & -\sin \theta\\ \sin \theta & \cos \theta \end{bmatrix}.
\end{equation*}
From this definition, we see that once $\mathbf{T}$ and $\mathbf{S}$ are known, the function $\theta$ can be computed by
\begin{equation*}
    \theta=\text{arg}(\mathbf{R}_1),
\end{equation*}
where $\mathbf{R}_1$ denotes the first column of $\mathbf{R}$. The orthonormalization technique and thus the choice of $\mathbf{T}$ influences the angle $\theta$. Our choice of $\mathbf{T}$ and the corresponding interpretation of $\theta$ is discussed in subsection \ref{sec:ChoiceTtheta}. \par
Defining $\mathbf{T}=(T_{ij})_{1\leq i,j \leq 2}$ and $\mathbf{T}^{-1}=(T^{ij})_{1\leq i,j \leq 2}$, and letting 
\begin{equation*}
    \mathbf{V_{ij}}=\nabla (T_{i1})T^{1j}+\nabla (T_{i2})T^{2j},
\end{equation*}
then $\theta$ is determined by the following equation \cite[Eq. (65)]{monard2012a}:
\begin{equation}\label{eq:theta}
    \nabla \theta = \mathbf{F},
\end{equation}
with
\begin{equation*}
    \mathbf{F}=\frac{1}{2}(\mathbf{V_{12}}-\mathbf{V_{21}}-\mathcal{J}\nabla \log D),
\end{equation*}
$\mathcal{J}=\begin{bmatrix} 0 & -1\\ 1 & 0\end{bmatrix}$, and $D=(H_{11}H_{22}-H_{12}^2)^{\frac{1}{2}}$. Once $\theta$ is known at at least one point on the boundary one can integrate $\mathbf{F}$ along curves originating from that point to obtain $\theta$ throughout the whole domain. Alternatively, when assuming that $\theta$ is known along the whole boundary one can apply the divergence operator to \eqref{eq:theta} and solve the following Poisson equation with Dirichlet boundary condition:
\begin{equation}\label{eq:thetaBVP}
    \begin{cases}
        \Delta \theta=\nabla \cdot \mathbf{F} & \text{in }\Omega,\\
        \theta=\theta_{\text{true}} & \text{on }\partial \Omega.
    \end{cases}
\end{equation}
In our implementation, we use the second option and discuss in subsection \ref{sec:ChoiceTtheta} knowledge of $\theta$ along the boundary.

\subsection{Reconstruction of $\sigma$}
Reconstruction of $\sigma$ is based on \cite[Eq. (68)]{monard2012a}
\begin{equation}\label{eq:sigmaRec}
    \nabla \log \sigma = \mathbf{G},
\end{equation}
with 
\begin{align*}
    \mathbf{G}&=\cos(2 \theta)\mathbf{K} + \sin(2\theta)\mathbf{K},\\
    \mathbf{K}&=\mathcal{U}(\mathbf{V_{11}}-\mathbf{V_{22}})+\mathcal{J}\mathcal{U}(\mathbf{V_{12}}-\mathbf{V_{21}}) \quad \text{and} \quad \mathcal{U}=\begin{bmatrix} 1 & 0\\ 0 & -1\end{bmatrix}.
\end{align*}
Similarly as for $\theta$ one need to solve a gradient equation to obtain $\sigma$ and has the possibility of either integrating along curves or solving a Poisson equation, assuming knowledge of $\sigma$ in one point or along the whole boundary respectively. We assume knowledge of $\sigma$ along the whole boundary and solve the following Poisson equation with Dirichlet condition:
\begin{equation}\label{eq:sigmaBVP}
    \begin{cases}
        \Delta \log (\sigma)= \nabla \cdot \mathbf{G} &\text{in }\Omega,\\
        \log (\sigma)=\log (\sigma_{\text{true}}) & \text{on }\partial \Omega.
    \end{cases}
\end{equation}

\subsection{Choice of the transfer matrix $\mathbf{T}$ and knowledge of $\theta$}
\label{sec:ChoiceTtheta}

For our implementation, we use Gram-Schmidt orthonormalization to obtain the transfer matrix $\mathbf{T}$:
\begin{equation*}
    \mathbf{T}=\begin{bmatrix} H_{11}^{-\frac{1}{2}} & 0 \\ -H_{12}H_{11}^{-\frac{1}{2}}D^{-1} & H_{11}^{\frac{1}{2}}D^{-1}\end{bmatrix}.
\end{equation*}
By the Jacobian constraint, it follows that $H_{11}>0$ so that $\mathbf{T}$ is well-defined. As a direct consequence of using Gram-Schmidt orthonormalization the first column of $\mathbf{R}$ simplifies to:
\begin{equation*}
    \mathbf{R}_1 = T_{11}\mathbf{S}_1 + T_{12} \mathbf{S}_2 = \frac{\cancel{\sqrt{\sigma}}\nabla u_1}{\cancel{\sqrt{\sigma}}\abs{\nabla u_1}}.
\end{equation*}
Therefore, the angle $\theta$ simply defines the angle between $\nabla u_1$ and the $x_1$-axis. Hence,
\begin{equation}\label{eq:thetau1}
    \theta = \text{arg}(\nabla u_1).
\end{equation}
In addition, following this definition for $\mathbf{T}$ the vector fields $\mathbf{V_{ij}}$ can be written explicitly in terms of $\mathbf{H}$:
\begin{align}\label{eq:Vexp}
\begin{aligned}
    \mathbf{V_{11}}&= \nabla \log H_{11}^{-\frac{1}{2}}, & \mathbf{V_{12}}&=0,\\ \mathbf{V_{21}}&= -\frac{H_{11}}{D} \nabla \left( \frac{H_{12}}{H_{11}}\right), & \mathbf{V_{22}}&=\nabla \log \left( \frac{H_{11}^{\frac{1}{2}}}{D}\right).
    \end{aligned}
\end{align}
Knowledge of $\theta$ at the boundary is essential for the reconstruction procedure. By this definition of $\mathbf{T}$, knowledge of $\theta$ is directly related to knowledge of the gradient $\nabla u_1$ and the current $\sigma \nabla u_1$, as both vector fields have the same direction. We decompose $\sigma \nabla u_1$ into two parts with contribution from the unit outward normal $\nu$ and the tangent vector $\omega=\mathcal{J}\nu$:
\begin{equation*}
    \sigma \nabla u_1 = (\sigma \nabla u_1 \cdot \nu)\nu + (\sigma \nabla u_1 \cdot \omega)\omega.
\end{equation*}
As along the whole boundary $u_1$ and $\sigma$ are known, the contribution from $\sigma \nabla u_1 \cdot \omega$ is known as well. Furthermore, along the part of the boundary $\partial \Omega \backslash \Gamma$ we have additional information as $u_1$ vanishes. Therefore, the only contribution is from the unit outward normal $\nu$, so that on this part of the boundary $\sigma \nabla u_1$ has either the direction of $\nu$, $-\nu$ or the zero vector. However, in order to have full information of $\theta$ along the boundary one needs knowledge about the Neumann data $\sigma \nabla u_1 \cdot \nu$.

\fi

\section{Numerical examples}
In this section we want to illustrate how boundary functions can be chosen in accordance with Theorem \ref{thm:Main} and how such functions work in practice to generate suitable AET measurements. We test the "suitability" of the measurements by numerically reconstructing the conductivity from this data following the analytic reconstruction procedure in section \ref{sec:recproc}. For that purpose, we have implemented the reconstruction procedure in section \ref{sec:recproc} in \python{} and use \fenics{}~\cite{fenics} to solve the PDEs. We use a fine mesh to generate our power density data and a coarser mesh to address the reconstruction problem. We use $N_{\text{data}}=79527$ nodes in the high-resolution case, while for the coarser mesh we consider a resolution of $N_{\text{recon}}=50925$ nodes. For both meshes, we use $\mathbb{P}_1$ elements. We consider our domain $\Omega$ to be the unit disk $B(0,1) \subset \R^2$ so that the boundary curve can be parameterized by $\eta:[0,2\pi] \rightarrow \partial \Omega$ as follows:
\begin{equation*}
    \eta(t)=arg(\cos(t)+i \sin(t)).
\end{equation*}
We consider 8 limited view settings for $\Gamma_i=\eta([0,\ell_i])$ ranging from $\ell_1=\frac{\pi}{4}$ to the full boundary with $\ell_8=2\pi$:
\begin{equation}\label{eq:Gam}
    \Gamma_i=\eta([0,\ell_i]) \quad \text{with} \quad \ell_i=i \frac{\pi}{4}, \quad \text{for} \quad i=1,..,8.
\end{equation}
We choose 8 sets of boundary functions for this limited view setting in accordance with Theorem \ref{thm:Main} so that $\abs{\mathrm{Ind}(\gamma(t))}=\abs{\mathrm{Ind}(f_{1,\mathrm{adapt}}^{\ell_i},f_{2,\mathrm{adapt}}^{\ell_i})}=1$. These functions are the coordinate functions $(\cos(\eta(t)),\sin(\eta(t)))$ adapted to the interval $[0,\ell_i]$:

\begin{equation} \label{eq:fadapt}
(f_{1,\mathrm{adapt}}^{\ell_i},f_{2,\mathrm{adapt}}^{\ell_i})=\begin{cases}
        (\cos(8\eta(t)),\sin(8\eta(t))) & t \in \lb 0,\ell_1 \rb\\
        (\cos(4\eta(t)),\sin(4\eta(t))) & t \in \lb 0,\ell_2 \rb\\
        \lp \cos \lp \frac{8}{3}\eta(t)\rp,\sin \lp\frac{8}{3}\eta(t)\rp \rp & t \in \lb 0,\ell_3 \rb\\
        \lp \cos \lp 2\eta(t)\rp,\sin \lp 2\eta(t)\rp \rp & t \in \lb 0,\ell_4 \rb\\
        \lp \cos \lp \frac{8}{5}\eta(t)\rp,\sin \lp\frac{8}{5}\eta(t)\rp \rp & t \in \lb 0,\ell_5 \rb\\
        \lp \cos \lp \frac{4}{3}\eta(t)\rp,\sin \lp\frac{4}{3}\eta(t)\rp \rp & t \in \lb 0,\ell_6 \rb\\
        \lp \cos \lp \frac{8}{7}\eta(t)\rp,\sin \lp\frac{8}{7}\eta(t)\rp \rp & t \in \lb 0,\ell_7 \rb\\
        (\cos(\eta(t)),\sin(\eta(t))) & t \in \lb 0,\ell_8 \rb
    \end{cases}
\end{equation}

These are illustrated in the first column of Figure \ref{fig:funs}. Additionally we choose 8 pairs of boundary function that corresponds to cut offs of the coordinate functions as in Remark \ref{rem:corrdcut}. These are so that $\abs{\mathrm{Ind}(\gamma(t))}=\abs{\mathrm{Ind}(f_{1,\mathrm{coord}}^{\ell_i},f_{2,\mathrm{coord}}^{\ell_i})}=\frac{i}{8}$:
\begin{equation}\label{eq:fcoord}
    (f_{1,\mathrm{coord}}^{\ell_i},f_{2,\mathrm{coord}}^{\ell_i})=\begin{cases}
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_1 \rb\\
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_2 \rb\\
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_3 \rb\\
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_4 \rb\\
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_5 \rb\\
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_6 \rb\\
        (\cos(\eta(t)),\sin(\eta(t)))- & t \in \lb 0,\ell_7 \rb\\
        (\cos(\eta(t)),\sin(\eta(t))) & t \in \lb 0,\ell_8\rb
    \end{cases}
\end{equation}
These are illustrated in the second column of Figure \ref{fig:funs}.

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/f1adapted.pdf}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Coord/f1coord.pdf}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Adapted/f2adapted.pdf}
        \caption*{Boundary functions as in equation \eqref{eq:fadapt}.}
        %\label{fig:f1a}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Coord/f2coord.pdf}
        \caption*{Boundary functions as in equation \eqref{eq:fcoord}.}
    \end{minipage}
    \caption{}
    \label{fig:funs}
\end{figure}
We consider two different phantoms; a piecewise constant phantom and a smooth phantom given explicitly by:
\begin{align}\label{eq:sig1}
    \sigma_{\text{1}}(x_1,x_2) &= \begin{cases}2 & \left(x_1+\frac{1}{2} \right)^2 + (x_2)^2 \leq 0.3^2,\\
        2 & \left(x_1\right)^2 + \left(x_2+\frac{1}{2} \right)^2 \leq 0.1^2,\\
        2 & \left(x_1-\frac{1}{2} \right)^2 + \left(x_2-\frac{1}{2} \right)^2 \leq 0.1^2,\\
        1 & \text{otherwise}.
    \end{cases}\\\label{eq:sig2}
    \sigma_{\text{2}}(x_1,x_2) &= \begin{cases}1 + e^{\left(2\,-\,\frac{2}{1-\frac{(x_1)^2+(x_2)^2}{1-0.8^2}}\right)} & 0\leq (x_1)^2+(x_2)^2 \leq 0.8^2,\\
    1 & 0.8^2 \leq (x_1)^2+(x_2)^2 \leq 1,
    \end{cases}
\end{align}
and illustrated in Figure \ref{fig:phantoms}.

\begin{figure}
    \centering
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{Figures2/TrueSigma.pdf}
        \caption*{$\sigma_{\text{1}}$}
    \end{minipage}%
    \begin{minipage}[t]{0.5\textwidth}
        \centering
        \includegraphics[width=\textwidth]{AdaptedPhantom2/TrueSigma2.pdf}
        \caption*{$\sigma_{\text{2}}$}
    \end{minipage}
    \caption{The true conductivities as in equations \eqref{eq:sig1} and \eqref{eq:sig2}.}
    \label{fig:phantoms}
\end{figure}
We solve the boundary value problem \eqref{condeqlim} in \fenics{} for these two different conductivities and the different boundary functions in equations \eqref{eq:fadapt} and \eqref{eq:fcoord} to generate power densities. To get an idea of how much information about the conductivity is captured in $H_{11}, H_{12}$ and $H_{22}$ for the two different choices of boundary functions, we illustrate the logarithm of these functions for the limited view setting $\Gamma_4=\eta([0,\pi])$ in Figure \ref{fig:Hijs}. The red line highlights the boundary of control $\Gamma$. As $H_{12}$ holds both positive and negative values we use the following bi-symmetric transformation:
\begin{equation}\label{logsym}
    \log_{\mathrm{sym}}(x) = \mathrm{sign}(x) \log \lp 1+\abs{\frac{x}{C}} \rp
\end{equation}
we use $C=10^{-3}$. This formula is based on \cite[eq.(4)]{webber2013a}. The upper row in Figure \ref{fig:Hijs} shows $H_{11}, H_{12}$ and $H_{22}$ corresponding to the adapted boundary functions in equation \eqref{eq:fadapt}. $H_{11}$ and $H_{22}$ visualize how the boundary conditions $f_{1,\text{adapt}}$ and $f_{2,\text{adapt}}$ illuminate the domain from different angles and thus capture different bits of information about the conductivity. The cross correlation $H_{12}$ then holds additional information from both boundary conditions combined. The edges of the inclusions are clearly visible close to the boundary of control $\Gamma$ and more faded away from $\Gamma$. Similar observations can be made about the second row in Figure \ref{fig:Hijs} corresponding to the cut off coordinate functions as boundary conditions in equation \eqref{eq:fadapt}. The main difference is that here the illuminated direction in $H_{11}$ for the adapted boundary functions roughly corresponds to the illuminated direction in $H_{22}$ and the same trend for $H_{22}$ for the adapted boundary functions roughly corresponds to the illuminated direction in $H_{11}$. Visually the information stored for both types of boundary functions seems similar. However, as the adapted boundary functions have more oscillations this may play a bigger role for really small boundaries, where these may succeed better at illuminating the domain. 


\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/AdaptH11}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/AdaptH12}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/AdaptH22}
        %\caption*{10\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/CoordH11}
        \caption*{$\log(H_{11})$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/CoordH12}
        \caption*{$\log_{\mathrm{sym}}(H_{12})$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureHijs/CoordH22}
        \caption*{$\log(H_{22})$}
    \end{minipage}
    \caption{Log plots of the power densities in case of adapted boundary functions as in eq. \eqref{eq:fadapt} (upper row) and cut off boundary functions as in eq. \eqref{eq:fcoord} (lower row). The true conductivity is $\sigma_1$. As $H_{12}$ holds both positive and negative values we use the bi-symmetric transformation $\log_{\mathrm{sym}}$ in \eqref{logsym}.}
    \label{fig:Hijs}
\end{figure}


\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures2/PlaceholderHijs2.png}
    \caption{Log plots of the power densities in case of adapted boundary functions as in eq. \eqref{eq:fadapt} (upper row) and cut off boundary functions as in eq. \eqref{eq:fcoord} (lower row). The true conductivity is $\sigma_1$. As $H_{12}$ holds both positive and negative values we use the bi-symmetric transformation $\log_{\mathrm{sym}}$ in \eqref{logsym}.}
    \label{fig:Hijs}
\end{figure}
\fi

In order to also illustrate the effect of the size of the boundary of control on the information captured in the power densities we show the logarithm of $H_{11}$ corresponding to the adapted boundary functions for the different limited view settings in Figure \ref{fig:H11s}. The edges of the conductivity are clearly visible for the full boundary of control and fade slowly away for decreasing size of $\Gamma$. Until for the smallest boundary $\Gamma_1$ only a little bit of the small inclusion close to $\Gamma_1$ is visible.

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11full}
        \caption*{$\Gamma_8$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11Huge}
        \caption*{$\Gamma_7$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11Lar}
        \caption*{$\Gamma_6$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11MedLar}
        \caption*{$\Gamma_5$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11Med}
        \caption*{$\Gamma_4$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11SmaMed}
        \caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11Sma}
        \caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureH11s/H11Mini}
        \caption*{$\Gamma_1$}
    \end{minipage}
    \caption{Log plots of the power density $H_{11}$ corresponding to the adapted boundary functions in eq. \eqref{eq:fadapt} and various sizes of the boundary of control $\Gamma$ (indicated by the red line). The true conductivity is $\sigma_1$.}
    \label{fig:H11s}
\end{figure}

In order to check the Jacobian condition \eqref{eq:nonvan} and the influence of the size of the boundary of control we illustrate the logarithm of $\det(\mathbf{H})=\sigma\det([\nabla u_1 \, \nabla u_2])^2$ in Figure \ref{fig:dets}. As the conductivity $\sigma_1$ takes values between 1 and 2 small values of $\det(\mathbf{H})$ correspond to small values of the Jacobian $\det([\nabla u_1 \, \nabla u_2])$. For the full boundary of control the small values of the Jacobian are centered around the inclusions and for the limited view settings all smallest values lie towards $\partial \Omega \setminus \Gamma$. This is in accordance with Remark \ref{rem:vio}. For decreasing size of $\Gamma$ the values of $\det(\mathbf{H})$ decrease and especially for the small boundaries of control, $\Gamma_1$ and $\Gamma_2$, almost the whole domain is corrupted by really small values of $\det(\mathbf{H})$ and thus the Jacobian.

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetFull}
        \caption*{$\Gamma_8$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetHuge}
        \caption*{$\Gamma_7$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetLar}
        \caption*{$\Gamma_6$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetLar}
        \caption*{$\Gamma_5$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetMed}
        \caption*{$\Gamma_4$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetSmaMed}
        \caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetSma}
        \caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureDets/DetMini}
        \caption*{$\Gamma_1$}
    \end{minipage}
    \caption{Log plots of $\det(\mathbf{H})=\sigma\det([\nabla u_1 \, \nabla u_2])^2$ corresponding to the adapted boundary functions in eq. \eqref{eq:fadapt} and various sizes of the boundary of control $\Gamma$ (indicated by the red line). The true conductivity is $\sigma_1$.}
    \label{fig:dets}
\end{figure}

Using the generated power densities we follow the procedure in section \ref{sec:recproc} to reconstruct $\sigma$. As there is no visual difference using the adapted boundary functions in equation \eqref{eq:fadapt} or the cut offs of the coordinate functions in \eqref{eq:fcoord} we only illustrate the reconstructions using the adapted boundary functions. Figure \ref{fig:sigmaRecs1} shows the reconstructions of $\sigma_1$ for varying sizes of $\Gamma$ and Figure \ref{fig:sigmaRecs2} shows the reconstructions of $\sigma_2$. For the full boundary of control we almost get perfect reconstructions in both cases (relative errors...). With decreasing size of $\Gamma$ the quality of the reconstruction decreases. Essentially the light areas of the function $H_{11}$ in Figure \ref{fig:H11s} that still capture a lot of information about the conductivity are also the areas for which one gets a good reconstruction. In particular the shape of the dark regions for the small boundaries of control, $\Gamma_1$ and $\Gamma_2$, are exactly the shapes that reappear as shadows in the reconstruction, where the reconstructed values are close to zero and thus way below the actual values between 1 and 2. While the reconstructed values for $\Gamma_1$ and $\Gamma_2$ are too small towards the boundary $\partial \Omega \setminus \Gamma_i$, the reconstructed values for the limited view settings $\Gamma_i$ for $i=3,...,7$ are too large towards this part of the boundary. And there seems to happen a transition from $\Gamma_3$ to $\Gamma_2$ where the quality of the reconstruction drops significantly, so this seems to be the point where the boundary of control is too small in order to have enough information for reconstruction when using the procedure in section \ref{sec:recproc}. The reconstruction performance is relatively similar for both conductivities apart from the fact that for the piecewise constant inclusions in $\sigma_1$ the reconstructed value even changes within the inclusions (as can be seen particularly for the boundaries of control $\Gamma_3$ and $\Gamma_4$). For the smooth feature in $\sigma_2$ the reconstructed value is the same for each limited view setting.


\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptFull}
        \caption*{$\Gamma_8$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptHuge}
        \caption*{$\Gamma_7$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptLar}
        \caption*{$\Gamma_6$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptMedLar}
        \caption*{$\Gamma_5$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptMed}
        \caption*{$\Gamma_4$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptSmaMed}
        \caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptSma}
        \caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptMini}
        \caption*{$\Gamma_1$}
    \end{minipage}
    \caption{Reconstructions when using the adapted boundary functions and various sizes of the boundary of control $\Gamma$ (indicated by the red line). The true conductivity is $\sigma_1$ and the colorbar corresponds to the one in Figure \ref{fig:phantoms}.}
    \label{fig:sigmaRecs1}
\end{figure}



\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures2/PlaceholderRecs.png}
    \caption{Reconstructions when using the adapted boundary functions and various sizes of the boundary of control $\Gamma$ (indicated by the red line). The true conductivity is $\sigma_1$ and the colorbar corresponds to the one in Figure \ref{fig:phantoms}.}
    \label{fig:sigmaRecs1}
\end{figure}
\fi



\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptFull}
        %\vspace{-5mm}
        \caption*{$\Gamma_8$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptHuge}
        \caption*{$\Gamma_7$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptLar}
        \caption*{$\Gamma_6$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptMedLar}
        \caption*{$\Gamma_5$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptMed}
        \caption*{$\Gamma_4$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptSmaMed}
        \caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptSma}
        \caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigurePhantom2/AdaptMini}
        \caption*{$\Gamma_1$}
    \end{minipage}
    \caption{Reconstructions when using the adapted boundary functions and various sizes of the boundary of control $\Gamma$ (indicated by the red line). The true conductivity is $\sigma_2$ and the colorbar corresponds to the one in Figure \ref{fig:phantoms}.}
    \label{fig:sigmaRecs2}
\end{figure}


\begin{table}[ht!]
    \centering
    \caption{Relative $L^2$ errors of $\sigma_1$ for the adapted and cut off boundary functions for varying sizes of $\Gamma$.}
    \begin{tabular}{c||c | c}
         & Adapted functions & Cut off functions\\ \hline \hline
         $\Gamma_8$ & 2.29\% & 2.29\%\\
         $\Gamma_7$ & 21.6\% & 21.2\%\\
         $\Gamma_6$ & 37.5\% & 38.0\% \\
         $\Gamma_5$ & 48.4\% & 49.3\% \\
         $\Gamma_4$ & 52.4\% & 46.1\% \\
         $\Gamma_3$ & 39.9\% & 28.8\% \\
         $\Gamma_2$ & 43.3\% & 55.5\% \\
         $\Gamma_1$ & 84.8\% & 87.1\% \\ \hline
    \end{tabular}
    \label{tab:sig1}
\end{table}

\begin{table}[ht!]
    \centering
    \caption{Relative $L^2$ errors of $\sigma_2$ for the adapted and cut off boundary functions for varying sizes of $\Gamma$.}
    \begin{tabular}{c||c | c}
         & Adapted functions & Cut off functions\\ \hline \hline
         $\Gamma_8$ & 0.03\% & 0.03\%\\
         $\Gamma_7$ & 22.1 \% & 21.2\%\\
         $\Gamma_6$ & 39.1 \% & 38.6\% \\
         $\Gamma_5$ & 51.0\% & 50.5\% \\
         $\Gamma_4$ & 54.0\% & 47.0\% \\
         $\Gamma_3$ & 39.5\% & 26.6\% \\
         $\Gamma_2$ & 37.3\% & 49.9\% \\
         $\Gamma_1$ & 76.2\% & 86.5\% \\ \hline
    \end{tabular}
    \label{tab:sig2}
\end{table}


\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.7cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/AdaptSmaMed.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/AdaptSmall.pdf}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/AdaptMini.pdf}
        %\caption*{10\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/CoordSmaMed.pdf}
        %\caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/CoordSmall.pdf}
        %\caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/CoordMini.pdf}
        %\caption*{$\Gamma_1$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ComparisonFigures/AsmaMedDiff.pdf}
        \caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ComparisonFigures/AsmaDiff.pdf}
        \caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ComparisonFigures/AminDiff.pdf}
        \caption*{$\Gamma_1$}
    \end{minipage}
    \caption{Comparing reconstructions of $\sigma_1$ when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs1compare}
\end{figure}

\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/AdaptSmaMed2.pdf}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/AdaptSmall2.pdf}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/AdaptMini2.pdf}
        %\caption*{10\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/CoordSmaMed2.pdf}
        %\caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/CoordSmall2.pdf}
        %\caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth,trim={2.8cm 1cm 2.5cm 1cm},clip]{ComparisonFigures/CoordMini2.pdf}
        %\caption*{$\Gamma_1$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ComparisonFigures/AsmaMedDiff2.pdf}
        \caption*{$\Gamma_3$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ComparisonFigures/AsmaDiff2.pdf}
        \caption*{$\Gamma_2$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \includegraphics[width=\linewidth]{ComparisonFigures/AminDiff2.pdf}
        \caption*{$\Gamma_1$}
    \end{minipage}
    \caption{Comparing reconstructions of $\sigma_2$ when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs2compare}
\end{figure}



\subsection{Reconstruction from noisy measurements}
We want to investigate 
\begin{equation*}
    \widetilde{H}_{ij} = H_{ij} + \frac{\alpha}{100} \frac{e_{ij}}{\norm{e_{ij}}_{L^2}} H_{ij},
\end{equation*}


\begin{figure}
    \centering
    \includegraphics[width=0.5\textwidth]{CoordNoise/TrueSigma.pdf}
    \caption{True conductivity $\sigma_1$ used for reconstruction from noisy measurements (note the difference in the range of the colorbar relative to Figure \ref{fig:phantoms}).}
    \label{fig:enter-label}
\end{figure}

%\begin{figure}[ht!]
%    \centering
%        \includegraphics[width=\linewidth]{Figures2/Noisefig.png}
%    \caption{Reconstructions for varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
%    \label{fig:sigmaRecs}
%\end{figure}


\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Adapt1noise}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Adapt5noise}
        %\caption*{5\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Adapt10noise}
        %\caption*{10\% noise, \lambda_{\min}=$10^{-6}$}
    \end{minipage}
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Coord1noise}
        \caption*{$1\%$ noise, $\lambda_{\min}=10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Coord5noise}
        \caption*{$5\%$ noise, $\lambda_{\min}=10^{-6}$}
    \end{minipage}%
    \begin{minipage}[t]{0.33\textwidth}
        \centering
        \input{TikzFigureNoise/Coord10noise}
        \caption*{$10\%$ noise, $\lambda_{\min}=10^{-6}$}
    \end{minipage}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs}
\end{figure}


\iffalse
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{Figures2/PlaceholderNoise2.png}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:enter-label}
\end{figure}
\fi


\iffalse
\begin{figure}[ht!]
    \centering
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigure/AdaptFull}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Huge}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Lar}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/MedLar}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Med}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/SmaMed}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Sma}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}%
    \begin{minipage}[t]{0.25\textwidth}
        \centering
        \input{TikzFigureCoord/Mini}
        %\caption*{1\% noise, \lambda_{\min}=$10^{-7}$}
    \end{minipage}
    \caption{Reconstructions when adding varying noise levels when using the adapted boundary functions (upper row) and the cut off of the coordinate functions (lower row).}
    \label{fig:sigmaRecs}
\end{figure}
\fi



%\begin{figure}
%    \centering
%    \includegraphics[width=\textwidth,trim={2.6cm 1.1cm 4cm 1.1cm},clip]{AdaptedNoise/ContMedNoise11e7.pdf}
%    \caption{Caption}
%    \label{fig:enter-label}
%\end{figure}
\clearpage

\section{Discussion}




\section{Acknowledgments}
H.S. was supported by the Research Council of Finland (Flagship of Advanced Mathematics for Sensing Imaging and Modelling grant 359208; Centre of Excellence of Inverse Modelling and Imaging grant 353092; and other grants 351656, 358047).

\clearpage

\iffalse

\section{Conclusions}
In this work, we have derived sufficient conditions on two boundary functions so that the corresponding solutions to the conductivity equation satisfy a non-vanishing Jacobian constraint in limited view. This approach allows for boundary functions that have discontinuities. This is relevant for Acousto-Electric Tomography and Current Density Imaging both in limited view and in full view settings, as the conditions and thus the use of discontinuous boundary functions apply for both settings. \par
We illustrated how these conditions could be used for numerical examples of reconstructing the conductivity from power density data in limited view following the approach of \cite{monard2012a}. It was evident from the numerical examples how the non-vanishing Jacobian constraint was almost violated close to the boundary that could not be controlled. This follows from the zero Dirichlet condition on this part of the boundary: Here the two corresponding solutions have both the direction of the unit normal so that the non-vanishing Jacobian constraint cannot be satisfied on this part of the boundary. Nevertheless, without noise it was possible to obtain decent reconstructions of the conductivity when the support of the boundary of control was at least half the size of the full boundary. For smaller boundaries of control the numerical results get unreliable due to small values of the Jacobian. Therefore in general it is almost impossible to add even small levels of noise while maintaining positive definiteness of the measurement matrix. To account for this, we used a small positive lower bound for the eigenvalues of the measurement matrix. This worked well in the numerical experiments even for high noise levels. However, in this approach especially values close to the part of the boundary that cannot be controlled are affected by the lower bound. When the lower bound is high this might be in contradiction with the assumption that values should be small in this region. This is especially a problem when using discontinuous boundary conditions as the lower bound needs to be chosen large when the noise level is high. \par
We mention that the proposed conditions in order to obtain solutions satisfying the non-vanishing Jacobian constraint are not optimal. Especially for the case of discontinuous boundary functions there is a possibility that \ref{thm:Main} (b) can be relaxed, as we are aware of functions that are more general than allowed here as indicated in Remark \ref{rem:Discont}.


\paragraph*{Acknowledgements}
The authors would like to express their sincere gratitude to our Nuutti Hyv\"onen for suggesting how to solve the boundary value problem \eqref{bvpui} numerically with discontinuous boundary conditions, and for providing the \matlab{} code to solve the boundary value problem \eqref{eq:LapBVP} semi-analytically as discussed in section \ref{sec:DBC}. M.S.\ was partly supported by the Academy of Finland (Centre of Excellence in Inverse Modelling and Imaging, grant 284715) and by the European Research Council under Horizon 2020 (ERC CoG 770924).
\fi
